Bayesian Optimization in a Billion Dimensions via Random Embeddings

Bayesian optimization techniques have been successfully applied to robotics, planning, sensor placement, recommendation, advertising, intelligent user interfaces and automatic algorithm configuration. Despite these successes, the approach is restricted to problems of moderate dimension, and several workshops on Bayesian optimization have identified its scaling to high-dimensions as one of the holy grails of the field. In this paper, we introduce a novel random embedding idea to attack this problem. The resulting Random EMbedding Bayesian Optimization (REMBO) algorithm is very simple, has important invariance properties, and applies to domains with both categorical and continuous variables. We present a thorough theoretical analysis of REMBO. Empirical results confirm that REMBO can effectively solve problems with billions of dimensions, provided the intrinsic dimensionality is low. They also show that REMBO achieves state-of-the-art performance in optimizing the 47 discrete parameters of a popular mixed integer linear programming solver.

==> embedding_arxiv/bayesianoptimization.tex <==
%!TEX root = embedding.tex

As mentioned in the introduction, Bayesian optimization has two ingredients that need to be specified: The prior and the acquisition function. In this work, we adopt GP priors. We review GPs very briefly and refer the interested reader to the book by \citeA{Rasmussen:2006}.
A GP is a distribution over functions specified by its mean function $m(\cdot)$ and covariance $k(\cdot,\cdot)$. More specifically, given a set of points $\vx_{1:t}$, with $\vx_i \in \mathbb{R}^D$, we have 
$$
\vf(\vx_{1:t}) \sim \mathcal{N}(\vm(\vx_{1:t}), \vK(\vx_{1:t}, \vx_{1:t})),
$$
where $\vK(\vx_{1:t}, \vx_{1:t})_{i,j} = k(\vx_i, \vx_j)$
serves as the covariance matrix. A common choice of $k$ is the squared exponential function (see Definition~\ref{def:sekernel} on page~\pageref{def:sekernel}),
but many other choices are possible depending on our degree of belief about the smoothness of the objective function.
%Note that $k(x, y) = 1$ when $x = y$ and as $\|x-y\|_2$ increases $k(x, y)$ decreases. This means that two points that are close %by have a bigger covariance and points that are far away from each other have smaller covariance. 

An advantage of using GPs lies in their analytical tractability. In particular, given observations $\vx_{1:t}$ with corresponding values $\vf_{1:t}$, where $f_i = f(\vx_i)$,  and a new point $\vx^{*}$, the joint distribution is given by:
$$
\begin{bmatrix}\vf_{1:t} \\
f^* \end{bmatrix} \sim \mathcal{N}\left( 
\begin{bmatrix}\vm(\vx_{1:t}) \\
m^* \end{bmatrix},  
\begin{bmatrix}
\vK(\vx_{1:t}, \vx_{1:t}) & \vk(\vx_{1:t}, \vx^*)\\
\vk(\vx^*, \vx_{1:t}) & k(\vx^*, \vx^*)\end{bmatrix}\right).
$$
For simplicity, we assume that $\vm(\vx_{1:t}) = \mathbf{0}$ and $m^* = 0$. Using the Sherman-Morrison-Woodbury formula, 
one can easily arrive at the posterior predictive distribution:
$$
f^* | \data_t, \vx^* \sim \mathcal{N}(\mu(\vx^*|\data_t), \sigma(\vx^*|\data_t)),
$$
with data $\data_t = \{\vx_{1:t}, \vf_{1:t} \}$, and mean and variance
\begin{eqnarray}
\nonumber{}\mu(\vx^*|\data_t) & = & \vk(\vx^*, \vx_{1:t}) \vK(\vx_{1:t}, \vx_{1:t})^{-1} \vf_{1:t}\\
\nonumber{}\sigma(\vx^*|\data_t) & = & k(\vx^*, \vx^*)-\vk(\vx^*, \vx_{1:t}) \vK(\vx_{1:t},\vx_{1:t})^{-1} \vk(\vx_{1:t}, \vx^*).\end{eqnarray}
That is, we can compute the posterior predictive mean $\mu(\cdot)$ and variance $\sigma(\cdot)$ exactly for any point $\vx^*$.

At each iteration of Bayesian optimization, one has to re-compute the predictive mean and variance. These two quantities are used to construct the second ingredient of Bayesian optimization: The acquisition function. In this work, we report results for the expected improvement acquisition function~\cite{Mockus:1982,Vazquez:2011,Bull:2011}:
\[\nonumber{}u(\vx|\mathcal{D}_t)=\mathbb{E}(\max\{0,f_{t+1}(\vx) - f(\xbest)\} |\data_t).\]
In this definition, $\xbest = \argmax_{\vx \in \{\vx_{1:t} \} }f(\vx)$
is the element with the best objective value in the first $t$ steps of the optimization process. The next query is:
\[\nonumber{}\vx_{t+1} = \argmax_{\vx \in {\cal X}} u(\vx|\mathcal{D}_t).\]
Note that this utility favors the selection of points with high variance (points in regions not well explored) and points with high mean value (points worth exploiting). We also experimented with the UCB acquisition function \cite{Srinivas:2010,deFreitas:2012} and found it to yield similar results. The optimization of the closed-form acquisition function can be carried out by off-the-shelf numerical optimization procedures, such as DIRECT \cite{Jones:1993} and CMA-ES~\cite{Hansen:2001:CDS:1108839.1108843}; it is only based on the GP model of the blackbox function $f$ and does not require additional evaluations of $f$. 

The Bayesian optimization procedure is shown in Algorithm~\ref{alg:bo}. 
\begin{algorithm}
\caption{Bayesian Optimization}
\label{alg:bo}
\begin{algorithmic}[1]
{
\STATE Initialize $\mathcal{D}_{0}$ as $\emptyset$.
\FOR{$t=1,2,\dots$}
  \STATE Find $\vx_{t+1}\! \in\! \mathbb{R}^D$ by optimizing the acquisition function $u$: $\vx_{t+1} \!= \!\argmax_{\vx \in {\cal X}} u(\vx|\mathcal{D}_t).$ 
  \STATE Augment the data $\mathcal{D}_{t+1} = \mathcal{D}_{t} \cup \{(\vx_{t+1}, f(\vx_{t+1}))\}$.
  \STATE Update the kernel hyper-parameters.
\ENDFOR
}
\end{algorithmic}
\end{algorithm}




==> embedding_arxiv/conclusion.tex <==
We have demonstrated that it is possible to use random embeddings in Bayesian optimization to optimize functions 
of extremely high extrinsic dimensionality $D$ provided that they have low intrinsic dimensionality $d_e$. 
%
Moreover, our resulting REMBO algorithm is coordinate independent %and has provable regret bounds that are independent of the extrinsic dimensionality $D$.
and it only requires a simple modification of the original Bayesian optimization algorithm; namely multiplication by a random matrix. 
%
We proved REMBO's independence of $D$ theoretically and empirically validated it by optimizing low-dimensional functions embedded in previously untenable extrinsic dimensionalities of up to $1$ billion. We also theoretically and empirically showed REMBO's rotational invariance.
%
Finally, we demonstrated that REMBO achieves state-of-the-art performance for optimizing the 47 discrete parameters of a popular mixed integer programming solver,
thereby providing further evidence for the observation (already put forward by Bergstra, Hutter and colleagues) that, for many problems of great practical interest, the number of important dimensions indeed appears to be much lower than their extrinsic dimensionality. 

% \textcolor{red}{
We note that the central idea of our work -- using an otherwise unmodified optimization procedure in a randomly embedded space -- in principle could be applied to arbitrary optimization procedures. Evaluating the effciency of this technique for other procedures is an interesting topic for future work.
% }
%Last but not least, we have shown that regardless of the extrinsic dimensionality of a function, one can optimize it efficiently such that simple regret vanishes at a rate that depends only on the effective dimensionality of the function.
% We have shown that by using random embedding we can efficiently optimize high dimensional functions, provided they have low effective dimensionality. 

% Studying convergence, etc.


==> embedding_arxiv/firstproof.tex <==

\begin{proof}
Since $f$ has effective dimensionality $d_e$, there exists an effective subspace ${\cal T} \subset \mathbb{R}^D$, such that rank$({\cal T}) = d_e$. Furthermore, any $\vx \in \mathbb{R}^D$ decomposes as
 $\vx = \vx_{\top} + \vx_{\bot}$, where $\vx_{\top} \in {\cal T}$ and $\vx_{\bot} \in {\cal T}^{\bot}$. Hence, $f(\vx) = f(\vx_{\top} + \vx_{\bot}) = f(\vx_{\top}).$ Therefore, without loss of generality, it will suffice to show that for all $\vx_{\top} \in {\cal T}$, there exists a $\vy\in \mathbb{R}^d$ such that $f(\vx_{\top}) = f(\vA\vy)$.

Let $\vPhi \in \mathbb{R}^{D \times d_e}$ be a matrix, whose columns form an orthonormal basis for ${\cal T}$. Hence, for each $\vx_{\top} \in {\cal T}$, there exists a $\vc \in \mathbb{R}^{d_e}$ such that $\vx_{\top} = \vPhi \vc$. Let us for now assume that $\vPhi^{T}\vA$ has rank $d_e$. If $\vPhi^{T}\vA$ has rank $d_e$, there exists a $\vy$ such that $(\vPhi^{T}\vA)\vy=\vc$. The orthogonal projection of $\vA\vy$ onto ${\cal T}$ is given by 
\[ \vPhi \vPhi^T \vA \vy = \vPhi \vc = \vx_{\top}. \]
Thus $\vA\vy = \vx_{\top} + \vx'$ for some $\vx' \in {\cal T}^{\bot}$ since $\vx_{\top}$ is the projection $\vA\vy$ onto ${\cal T}$.
Consequently, $f(\vA\vy) = f(\vx_{\top} + \vx') = f(\vx_{\top})$. 

It remains to show that, with probability one, the matrix $\vPhi^T \vA$ has rank $d_e$.
Let $\vA_{e} \in \mathbb{R}^{D\times d_e}$ be a submatrix of $\vA$ consisting of any $d_e$ columns of $\vA$, which are \emph{i.i.d.} samples distributed according to $\mathcal{N}(\mathbf{0}, \vI)$. Then, $\vPhi^T \va_{i}$ are \emph{i.i.d.} samples from $\mathcal{N}(\mathbf{0}, \vPhi^T \vPhi) = \mathcal{N}(\mathbf{0}_{d_e}, \vI_{d_e\times d_e})$, and so we have $\vPhi^T\vA_e$, when considered as an element of $\mathbb{R}^{d_e^2}$, is a sample from $\mathcal{N}(\mathbf{0}_{d_e^2}, \vI_{d_e^2\times d_e^2})$. On the other hand, the set of singular matrices in $\mathbb{R}^{d_e^2}$ has Lebesgue measure zero, since it is the zero set of a polynomial (i.e. the determinant function) and polynomial functions are Lebesgue measurable. Moreover, the Normal distribution is absolutely continuous with respect to the Lebesgue measure, so our matrix $\vPhi^T \vA_e$ is almost surely non-singular, which means that it has rank $d_e$ and so the same is true of $\vPhi^T \vA$, whose columns contain the columns of $\vPhi^T \vA_e$.
\end{proof}


==> embedding_arxiv/hyper-parameter-optimization.tex <==
%!TEX root = embedding.tex
\begin{algorithm}[t]
\caption{Bayesian Optimization with Hyper-parameter Optimization.}
\label{alg:bohyper}
\begin{algorithmic}[1]
{
\INPUT Threshold $t_{\sigma}$.  
\INPUT Upper and lower bounds $U > L > 0$ for hyper-parameter. 
\INPUT Initial length scale hyper-parameter $\ell \in [L, U]$.
\STATE Initialize $C = 0$

\FOR{$t=1,2,\dots$}
  \STATE Find $\vx_{t+1}$ by optimizing the acquisition function $u$: $\vx_{t+1} = \argmax_{\vx \in {\cal X}} u(\vx|\mathcal{D}_t).$ 
  \IF{$\sqrt{\sigma^2(\vx_{t+1})} < t_{\sigma} $}
    \STATE $C = C + 1$
  \ELSE
    \STATE $C = 0$
  \ENDIF
  \STATE Augment the data $\mathcal{D}_{t+1} = \{\mathcal{D}_{t}, (\vx_{t+1}, f(\vx_{t+1})) \}$
  
  
  \IF{$t \mod 20 = 0$ \OR $C=5$}
    \IF{$C=5$}
        \STATE $U = \max\{0.9 \ell, L\}$
        \STATE $C = 0$
    \ENDIF
    \STATE Learn the hyper-parameter by optimizing the log marginal likelihood by using DIRECT and CMA-ES: $\ell=\argmax_{l \in [L, U]} \log p (\vf_{1:t+1}|\vx_{1:t+1}, l)$
  \ENDIF
\ENDFOR
}
\end{algorithmic}
\end{algorithm}

For Bayesian optimization (and therefore REMBO), it is difficult to manually estimate the true length scale hyper-parameter of a problem at hand. 
 To avoid any manual steps and to achieve robust performance across diverse sets of objective functions, in this paper we adopted an adaptive hyper-parameter optimization scheme. 
The length scale of GPs is often set by maximizing marginal likelihood~\cite{Rasmussen:2006,Jones:1998}. However, as demonstrated by \citeA{Bull:2011}, this approach, when implemented naively, may not guarantee convergence. This is not only true of approaches that maximize the marginal likelihood, but also of approaches that rely on Monte Carlo sampling from the posterior distribution \cite{Brochu:2010,Snoek:2012} when the number of data is very small, unless the prior is very informative.

Here, we propose to optimize the length scale parameter $\ell$ by maximizing the marginal likelihood subject to an upper bound $U$ which is decreased when the algorithm starts exploiting too much. 
Full details are given in Algorithm~\ref{alg:bohyper}.
We say that the algorithm is exploiting when the standard deviation at the maximizer of the acquisition function $\sqrt{\sigma(\vx_{t+1})}$ is less than some threshold $t_{\sigma}$ for $5$ consecutive iterations. 
Intuitively, this means that the algorithm did not emphasize exploration (searching in new parts of the space, where the predictive uncertainty is high) for $5$ consecutive iterations. When this criterion is met, the algorithm decreases its upper bound $U$ multiplicatively and re-optimizes the hyper-parameter subject to the new bound.
Even when the criterion is not met the hyper-parameter is re-optimized every $20$ iterations.
For each optimization of the acquisition function, the algorithm runs both DIRECT~\cite{Jones:1993} and CMA-ES~\cite{Hansen:2001:CDS:1108839.1108843} 
and uses the result of the best of the two options.
% \textcolor{magenta} {
The astute reader may wonder about the difficulty of optimizing the 
acquisition functions. For REMBO, however, we have not found the optimization of the acquisition function
to be a problem since we only need to optimize it in the low-dimensional space
and our acquisition function evaluations are cheap, allowing us tens of
thousands of evaluations in seconds that (empirically) suffice to cover the 
low-dimensional space well.
% }

The motivation of this algorithm is to rather err on the side of having too small a length scale:
% Our proof of Theorem~\ref{thm:regret} is based on the same concept: 
given a squared exponential kernel $k_\ell$, with a smaller length scale than another kernel $k$, one can show that any function $f$ in the RKHS characterized by $k$ is also an element of the RKHS characterized by $k_\ell$.
Thus, when running expected improvement, one can safely use $k_\ell$ instead of $k$ as the kernel of the GP and still preserve convergence~\cite{Bull:2011}. We argue that (with a small enough lower bound $L$) the algorithm would eventually reduce the upper bound enough to allow convergence.
Also, the algorithm would not explore indefinitely as $L$ is required to be positive.
%\note{FH: do we believe this argument will hold up to formal srutiny? Could we write it as a proposition and prove it?}
In our experiments, we set the initial constraint $[L, U]$ to be $[0.01, 50]$ and set $t_{\sigma} = 0.002$. 

% \textcolor{magenta} {
We want to stress the fact that the above argument
is only known to hold for a class of kernels over continuous domains (e.g.\ squared exponential and Mat\'ern class kernels). 
Although we believe that a similar argument could be made for
integer and categorical kernels, 
rigorous arguments concerning convergence under these kernels remain a challenge
in Bayesian optimization.
% }


==> embedding_arxiv/introduction.tex <==
%!TEX root = embedding.tex
Let $f: {\cal X} \to \mathbb{R}$ be a function on a compact subset ${\cal X} \subseteq \mathbb{R}^D$. We address the following global optimization problem
\[ \vx^{\star} = \argmax_{\vx \in {\cal X}} f(\vx). \]
We are particularly interested in objective functions $f$ that may satisfy one or more of the following criteria: they do not have a closed-form expression, are expensive to evaluate, do not have easily available derivatives, or are non-convex. We treat $f$ as a \emph{blackbox} function that only allows us to query its function value at arbitrary $x\in \cal{X}$.
To address objectives of this challenging nature, we adopt the Bayesian optimization framework. 

%\note{FH: I used this variant of text here, commenting out the text that used the term `risk function' (mixing nomenclature between risk and acquisition function was confusing).}
In a nutshell, in order to optimize a blackbox function $f$, Bayesian optimization uses a prior distribution that captures our beliefs about the behavior of $f$,
and updates this prior with sequentially acquired data.
Specifically, it iterates the following phases:
(1)~use the prior to decide at which input $x\in \cal X$ to query $f$ next; 
%; for example the expected improvement over the best function value seen so far); 
(2)~evaluate $f(x)$; and (3)~update the prior based on the new data $\langle{}x, f(x)\rangle$.
Step 1 uses a so-called \emph{acquisition function} that quantifies the expected value of learning the value of $f(x)$ for each $x \in \cal X$. This procedure is illustrated in Figure~\ref{Fig:BOpic}.
\begin{figure}[t]
\begin{center}
\includegraphics[width=13cm]{figures/toyGPtext3.pdf}
\end{center}
\caption{Three consecutive iterations of Bayesian optimization for a toy one-dimensional problem. The unknown objective function is approximated with at Gaussian process (GP) at each iteration. The figure shows the mean and confidence intervals for this process.
It also shows the acquisition function in the lower green shaded plots. The acquisition is high where the GP predicts a high objective (exploitation) and where the prediction uncertainty is high (exploration). 
Note that the area on the far left remains under-sampled, as (despite having high uncertainty) it is correctly predicted to be unlikely to improve over the highest observation.}
\label{Fig:BOpic}
\end{figure}



%Bayesian optimization methods differ in their choice of prior and their choice of this acquisition function.
%\note{FH: to make this journal paper self-contained, can we put in a figure for this, e.g. Figure 1 in \cite{Brochu:2009}?}
%
%Bayesian optimization has two ingredients. The first ingredient is a prior distribution that captures our beliefs about the behavior of the unknown objective function. The second ingredient is a risk function that describes the deviation from the global optimum. The expected risk is used to decide where to sample next. After observing a few samples of the objective, the prior is updated to produce a more informative posterior distribution over the space of objective functions \cite<see Figure 1 in>[]{Brochu:2009}.
%
%One problem with this maximum expected utility framework is that the risk is typically very hard to compute. This has led to the introduction of many sequential heuristics, known as acquisition functions, including Thompson sampling \cite{Thompson:1933}, probability of improvement \cite{Jones:2001}, expected improvement \cite{Mockus:1994} and upper-confidence-bounds \cite{Srinivas:2010}. 
The role of the acquisition function is to trade off exploration and exploitation; popular choices include Thompson sampling \cite{Thompson:1933,Hoffman:2014}, probability of improvement \cite{Jones:2001}, expected improvement \cite{Mockus:1994}, upper-confidence-bounds \cite{Srinivas:2010}, and online portfolios of these \cite{Hoffman:2011}.  
These are typically optimized by choosing 
points where the predictive mean is high (exploitation) and where the variance is large (exploration). Since they typically have an analytical expression that is easy to evaluate, they are much easier to optimize than the original objective function, using off-the-shelf numerical optimization algorithms.\footnote{This optimization step can in fact be circumvented when using treed multi-scale optimistic optimization as recently demonstrated by \citeA{Wang:2014}. There also exist several more involved Bayesian non-linear experimental design approaches for constructing the acquisition function, where the utility to be optimized involves an entropy of an aspect of the posterior. This includes the work of \citeA{Hennig:2012} for finding maxima of functions, the works of \citeA{Kueck:2006} and \citeA{Kueck:2009} for learning functions, and the work of \citeA{Hoffman:2009} for estimating Markov decision processes. These works rely on expensive approximate inference methods for computing intractable integrals.} 

The term \emph{Bayesian optimization} was coined several decades ago by Jonas Mo{\v c}kus \citeyear{Mockus:1982}. 
A popular version of the method is known as \emph{efficient global optimization} in the experimental design literature since the 
%nineties \cite{Schonlau:1998}. 
1990s \cite{Jones:1998}. 
Often, the approximation of the objective function is obtained using Gaussian process~(GP) priors. For this reason, the technique is also referred to as \emph{GP bandits} \cite{Srinivas:2010}. However, many other approximations of the objective have been proposed, including Parzen estimators \cite{Bergstra:2011}, Bayesian parametric models \cite{Wang:2011}, treed GPs \cite{Gramacy:2004} and random forests \cite{Brochu:2009,Hutter:2009,Hutter:2011}. 
%\note{FH: for me: check that ref.}
These may be more suitable than GPs when the number of iterations grows without bound, or when the objective function is believed to have discontinuities. We also note that often assumptions on the smoothness of the objective function are encoded without use of the Bayesian paradigm, while leading to similar algorithms and theoretical guarantees \cite<see, for example,>[and the references therein]{Bubeck:2011}.
%
There is a rich literature on Bayesian optimization, and for further details we refer readers to more tutorial treatments \cite{Brochu:2009,Jones:1998,Jones:2001,Lizotte:2011,Mockus:1994,Osborne:2009} and recent theoretical results~\cite{Srinivas:2010,Bull:2011,deFreitas:2012}. 


Bayesian optimization has been demonstrated to outperform other state-of-the-art blackbox optimization techniques when function evaluations are expensive and the number of allowed function evaluations is therefore low~\cite{HutHooLey13:BBOB}. In recent years, it has found increasing use in the machine learning community~\cite{Rasmussen:2003,Brochu:2007,martinez-cantin:2007,Lizotte:2008_IJCAI,Frazier:2009,Azimi:2010,Hamze:2011,Azimi:2011,Hutter:2011,Bergstra:2011,Gramacy:2011,Denil:2012,Mahendran:2012,Azimi:2012,Hennig:2012,Marchant:2012,Snoek:2012,Swersky:2013,Thornton:2013}. Despite many success stories, the approach is restricted to problems of moderate dimension, typically up to about 10. Of course, for a great many problems this is all that is needed. However, to advance the state of the art, we need to scale the methodology to high-dimensional parameter spaces. This is the goal of this paper.

It is difficult to scale Bayesian optimization to high dimensions. To ensure that a global optimum is found, we require good coverage of $\mathcal{X}$, but as the dimensionality increases, the number of evaluations needed to cover $\mathcal{X}$ increases exponentially. As a result, there has been little progress on this challenging problem, with a few exceptions.
%
\citeA{Bergstra:2011} introduced a non-standard Bayesian optimization method based on a tree of one-dimensional density estimators and applied it successfully to optimize the 238 parameters of a complex vision architecture \cite{Bergstra:model_search}.
%
\citeA{Hutter:2011} used random forests models in Bayesian optimization to achieve state-of-the-art performance in optimizing up to 76 mixed discrete/continuous parameters of algorithms for solving hard combinatorial problems, and to successfully carry out combined model selection and hyperparameter optimization for the 768 parameters of the Auto-WEKA framework~\cite{Thornton:2013}. 
%
\citeA{Eggensperger:2013} showed that these two methods indeed yielded the best performance for high-dimensional hyperparameter optimization (e.g., in deep belief networks). However, both are based on weak uncertainty estimates that can fail even for the optimization of very simple functions and lack theoretical guarantees. 
%Their software, which we benchmark against in our experiments, was the result of perhaps the most significant and non-trivial engineering endeavor in practical Bayesian optimization.

In the \emph{linear} bandits case, \citeA{Carpentier:2012} recently proposed a compressed sensing strategy to attack problems with a high degree of sparsity. 
Also recently, \citeA{Chen:2012} made significant progress by introducing a two stage strategy for optimization and variable selection of high-dimensional GPs. In the first stage, sequential likelihood ratio tests, with a couple of tuning parameters, are used to select the relevant dimensions. 
This, however, requires the relevant dimensions to be axis-aligned with an ARD kernel. Chen and colleagues provide empirical results only for synthetic examples (of up to 400 dimensions), but they provide key theoretical guarantees.

Many researchers have noted that for certain classes of problems most dimensions do not change the objective function significantly; examples include hyper-parameter optimization for neural networks and deep belief networks~\cite{Bergstra:2012}, as well as other machine learning algorithms and various state-of-the-art algorithms for solving $\mathcal{NP}$-hard problems~\cite{Hutter:2014}.
That is to say these problems have \emph{``low effective dimensionality''}. To take advantage of this property, \citeA{Bergstra:2012} proposed to simply use random search for optimization -- the rationale being that points sampled uniformly at random in each dimension can densely cover each low-dimensional subspace. As such, random search can exploit low effective dimensionality \emph{without knowing which dimensions are important}. In this paper, we exploit the same property in a new Bayesian optimization variant based on random embeddings. 
%In this paper, we show that random embeddings have the same property, and combine them with powerful Bayesian optimization in the low-dimensional subspace.



Figure \ref{fig:simple_embedding} illustrates the idea behind random embeddings in a nutshell.
Assume we know that a given $D=2$ dimensional black-box function $f(x_1, x_2)$ only has $d=1$ important dimensions, but we do not know which of the two dimensions is the important one.
We can then perform optimization in the embedded 1-dimensional subspace defined by $x_1=x_2$ since this is guaranteed to include the optimum. 

\begin{figure}[tb]
  \includegraphics[scale=0.32]{figures/2to1embedding.pdf}
  \centering
  \caption{This function in D=2 dimesions only has d=1 \emph{effective dimension}: the vertical axis indicated with the word important on the right hand side figure. Hence, the $1$-dimensional embedding includes the $2$-dimensional function's optimizer. It is more efficient to search for the optimum along the 1-dimensional random embedding than in the original 2-dimensional space.}
  \label{fig:simple_embedding}
\end{figure}

As we first demonstrated in a recent IJCAI conference paper~\cite{WangEtAl13}, random embeddings enable us to scale Bayesian optimization to arbitrary $D$ provided the objective function has low intrinsic dimensionality.
Importantly, the algorithm associated with this idea, which we called REMBO, is not restricted to cases with axis-aligned intrinsic dimensions but applies to any $d$-dimensional linear subspace. \citeA{Djolonga:2013} recently proposed an adaptive, but more expensive, variant of REMBO with theoretical guarantees.

In this journal version of our work, we expand the presentation to provide more details throughout.
%clarify some of the questions that arose following the publication of our IJCAI paper. 
In particular, we expand our description of the strategy for selecting the boundaries of the low-dimensional space and for setting the kernel length scale parameter; we show by means of an additional application (automatic configuration of random forest body-part classifiers) that the performance of our technique does not collapse when the problem does not have an obvious low effective dimensionality.
%  and we derive new theoretical bounds showing that under 
% certain
% %mild 
% assumptions the regret of our approach only depends on the problem's intrinsic dimensionality (Section \ref{sec:rembo}).
%
Our experiments (Section \ref{sec:experiments}) also show that REMBO can solve problems of previously untenable high extrinsic dimensions, and that REMBO can achieve state-of-the-art performance for optimizing the 47 discrete parameters of a popular mixed integer linear programming solver. 



%Section \ref{sec:conclusion} concludes the paper.


==> embedding_arxiv/journal-length-abstract-and-intro.tex <==
\begin{abstract}

Bayesian optimization is a powerful strategy for finding the extrema of objective functions. It is applicable in situations where one does not have a closed-form expression for the objective function, but where one can obtain noisy evaluations of this function at sampled values. It is particularly useful when these evaluations are costly, when one does not have access to derivatives, or when the problem at hand is non-convex. Bayesian optimization techniques have been successfully applied to robotics, planning, sensor placement, news recommendation, advertising, intelligent user interfaces and automatic algorithm configuration. Despite these successes, the approach is restricted to problems of moderate dimension. Several machine learning workshops on this topic have identified the scaling of Bayesian optimization to high-dimensions as a core challenge. Despite this, little progress has been made in this direction.
In this paper, we introduce a novel random embedding idea to scale Bayesian optimization to higher dimensions. The resulting algorithm is very simple, it has theoretical guarantees, it applies to domains with both categorical and continuous variables, and its hyper-parameters are automatically tuned. We show that the algorithm can effectively solve problems with billions of dimensions, provided the intrinsic dimensionality is low. We also show that it has important invariance properties. In terms of applications, we demonstrate that the algorithm performs remarkably well in the domains of automatic tuning of popular linear programming solvers and random forests classifiers for big data produced by the Kinect sensor.
\end{abstract}


\section{Introduction}
\label{sec:introduction}

Let $f: {\cal X} \to \mathbb{R}$ be a function on a compact subset ${\cal X} \subseteq \mathbb{R}^D$. We address the following global optimization problem
\[ \vx^{\star} = \argmax_{\vx \in {\cal X}} f(\vx). \]
We are particularly interested in objective functions $f$ that may satisfy any of the following criteria: Do not have a closed-form expression, are expensive to evaluate, are stochastic, do not have derivatives available, or are non-convex. For these reasons, we adopt the Bayesian optimization framework. We present a brief introduction to Bayesian optimization in this paper, but refer readers unfamiliar with the topic to more tutorial treatments \cite{Brochu:2009,Jones:1998,Jones:2001,Lizotte:2011,Mockus:1994,Osborne:2009}. 

Bayesian optimization has two ingredients. The first ingredient is a prior distribution that captures our beliefs about the behavior of the unknown objective function. The second ingredient is a risk function that describes the deviation from the global optimum. The expected risk is used to decide where to sample next. After observing a few samples of the objective, the prior is updated to produce a more informative posterior distribution over the space of objective functions \cite[see Figure 1 in][]{Brochu:2009}. One problem with this maximum expected utility framework is that the risk is typically very hard to compute. This has led to the introduction of many sequential heuristics, known as acquisition functions, including Thompson sampling \cite{Thompson:1933}, probability of improvement \cite{Jones:2001}, expected improvement \cite{Mockus:1994} and upper-confidence-bounds \cite{Srinivas:2010}. These acquisition functions trade-off exploration and exploitation. They are typically optimized by choosing points 
where the predictive mean is high (exploitation) and where the variance is large (exploration). Since the acquisition function has an analytical expression that is easy to evaluate, it is much easier to optimize than the original objective function, using algorithms such as DIRECT \cite{Finkel:2003} or projected Newton methods \cite{Bertsekas:1987}. It is also possible to use dynamic portfolios of acquisition functions to improve the efficiency of the method \cite{Hoffman:2011}. 

The term Bayesian optimization seems to have been coined several decades ago by Jonas Mo{\v c}kus \yrcite{Mockus:1982}. A popular version of the method has been known as efficient global optimization in the experimental design literature since the nineties \cite{Schonlau:1998}. Often, the approximation of the objective function is obtained using Gaussian process~(GP) priors. For this reason, the technique is also referred to as GP bandits \cite{Srinivas:2010}. However, many other approximations of the objective have been proposed, including Parzen estimators \cite{Bergstra:2011}, Bayesian parametric models \cite{Wang:2011}, treed GPs \cite{Gramacy:2004} and random forests \cite{Brochu:2009,Hutter:2009}. 
These may be more suitable than GPs when the number of iterations grows without bound, or when the objective function is believed to have discontinuities. We also note that often assumptions on the smoothness of the objective function are encoded without use of the Bayesian paradigm, while leading to similar algorithms and theoretical guarantees \cite[see, for example,][and the references therein]{Bubeck:2011,deFreitas:2012}.

In recent years, the machine learning community has increasingly used Bayesian optimization to optimize expensive objective functions. Despite many success stories, the approach is restricted to problems of moderate dimension, typically up to about 10. Of course, for a great many problems this is all that is needed. However, to advance the state of the art, we need to scale the methodology to high-dimensional parameter spaces. This is the goal of this paper.

It is difficult to scale Bayesian optimization to high dimensions. To ensure that a global optimum is found, we require good coverage of $\mathcal{X}$, but as the dimensionality increases, the number of evaluations needed to cover $\mathcal{X}$ increases exponentially. As a result, there has been little progress on this challenging problem, with a few exceptions.
%
%\note{NdF: Possibly revisit the following remark after experiments}
\citeA{Hutter:2011} used random forests models in Bayesian optimization to optimize up to 76 mixed discrete/continuous parameters of algorithms for solving hard combinatorial problems, empirically outperforming all competing algorithm configuration methods. However, their method is based on frequentist uncertainty estimates that can fail even for the optimization of very simple functions and lacks theoretical guarantees. Their software, which we benchmark against in our experiments, was the result of perhaps the most significant and non-trivial engineering endeavor in practical Bayesian optimization.
% the RFs are also axis-aligned, but that'll be better to mention in the context of the synthetic data experiment

In the \emph{linear} bandits case, \citeA{Carpentier:2012} recently proposed a compressed sensing strategy to attack problems with a high degree of sparsity. 
Also recently, Chen et al \citeA{Chen:2012} made significant progress by introducing a two stage strategy for optimization and variable selection of high-dimensional GPs. In the first stage, sequential likelihood ratio tests, with a couple of tuning parameters, are used to select the relevant dimensions. 
\note{FH: do we need ``with a couple of tuning parameters'' here? Seems to have a negative co-notation?}
This, however, requires the relevant dimensions to be axis-aligned with an ARD kernel. Chen et al provide empirical results only for synthetic examples (of up to 400 dimensions), but they provide key theoretical guarantees.

Many researchers have noted that for certain classes of problems most dimensions do not change the objective function significantly; examples include hyper-parameter optimization for neural networks and deep belief networks~\cite{Bergstra:2012} and automatic configuration of state-of-the-art algorithms for solving $\mathcal{NP}$-hard 
%problems~\cite{Hutter:2009}.
problems~\cite{Hutter:2013_key_parameters}.
%, and XXX~\cite{Caflisch:1997}. 
%\note{FH: TODO: what is the application domain in \cite{Caflisch:1997}??}
That is to say these problems have \emph{``low effective dimensionality''}. To take advantage of this property, \citeA{Bergstra:2012} proposed to simply use random search for optimization -- the rationale being that points sampled uniformly at random in each dimension can densely cover each low-dimensional subspace. As such, random search can exploit low effective dimensionality \emph{without knowing which dimensions are important}. In this paper, we exploit the same property in a new Bayesian optimization variant based on random embeddings. 
%In this paper, we show that random embeddings have the same property, and combine them with powerful Bayesian optimization in the low-dimensional subspace.


\begin{figure}[tb]
  \includegraphics[scale=0.16]{figures/2to1embedding.pdf}
  \centering
  \caption{This function only has one \emph{effective dimension}: the vertical axis indicated with the word important on the right hand side figure. Hence, the $1$D embedding includes the $2$D function's optimizer. It is more efficient to search for the optimum along the 1D random embedding than to conduct a grid-search in 2D.}
  \label{fig:simple_embedding}
\end{figure}

Figure \ref{fig:simple_embedding} illustrates the idea behind random embeddings in a nutshell.
Assume we know that a given $D=2$ dimensional black-box function $f(x_1, x_2)$ only has $d=1$ important dimensions, but we do not know which of the two dimensions is the important one.
We can then perform optimization in the embedded 1-dimensional subspace defined by $x_1=x_2$ since this is guaranteed to include the optimum. 
As we demonstrate in this paper, using random embeddings this simple idea largely scales to arbitrary $D$ and $d$, allowing us to perform
Bayesian optimization in a low-dimensional space to optimize a high-dimensional function with low intrinsic dimensionality.
Importantly, this trick is not restricted to cases with axis-aligned intrinsic dimensions but applies to any $d$-dimensional linear subspace.

After defining GP-based Bayesian optimization (Section \ref{sec:bo}), we describe Bayesian optimization based on random embeddings (REMBO) more formally and prove theoretical properties including regret bounds independent of $D$ (Section \ref{sec:rembo}). Then we demonstrate REMBO's empirical performance in a wide variety of settings (Section \ref{sec:experiments}). First, we evaluate scaling behaviour on synthetic data, demonstrating that REMBO can effectively optimize functions of low effective dimensionality embedded in a billion dimensions. Then, we demonstrate state-of-the-art performance for two real-world application domains: optimizing the 14 continuous parameters of a random forest classifier for body part classification using the Kinect sensor; and the 47 discrete parameters of a widely-used algorithm for solving mixed integer programs. 
%Section \ref{sec:conclusion} concludes the paper and points out promising directions for future work.


==> embedding_arxiv/linearProg.tex <==
%!TEX root = embedding.tex
State-of-the-art algorithms for solving hard computational problems tend to parameterize several design choices in order to allow a customization of the algorithm to new problem domains. Automated methods for algorithm configuration have recently demonstrated that substantial performance gains of state-of-the-art algorithms can be achieved in a fully automated fashion~\cite{Mockus:1999,ParamILS-JAIR,Hutter:2010,ValEtAl11,Bergstra:2011,Wang:2011}. 
%FH: HutBabHooHu07 would be a better ref, but too many self-citations...
These successes have led to a paradigm shift in algorithm development towards the 
active design of highly parameterized frameworks that can be automatically customized to particular problem domains using optimization~\cite{Hoos:2012:PO:2076450.2076469,Bergstra:model_search,Thornton:2013}.
%
The resulting algorithm configuration problems have been shown to have low dimensionality~\cite{Hutter:2014}, and here, we demonstrate that REMBO can exploit this low dimensionality even in the discrete spaces typically encountered in algorithm configuration. 
%
We use a configuration problem obtained from \citeA{Hutter:2010}, aiming to configure the 40 binary and 7 categorical parameters of \text{lpsolve}~\cite{lpsolve}
% \footnote{http://lpsolve.sourceforge.net/}
, a popular mixed integer programming (MIP) solver that has been downloaded over 40\,000 times in the last year.
The objective is to minimize the optimality gap \texttt{lpsolve} can obtain in a time limit of five seconds for a MIP encoding of a wildlife corridor problem from computational sustainability~\cite{ghs08:connection}.
Algorithm configuration usually aims to improve performance for a representative set of problem instances, and effective methods need to solve two orthogonal problems: searching the parameter space effectively and deciding how many instances to use in each evaluation (to trade off computational overhead and over-fitting). Our contribution is for the first of these problems; to focus on how effectively the different methods search the parameter space, we only consider configuration on a single problem instance.

Due to the discrete nature of this optimization problem, we could only apply REMBO using the high-dimensional kernel for categorical variables $k^D_{\lambda}(\vy^{(1)}, \vy^{(2)})$ described in Section \ref{sec:choice_of_kernel}. While we have not proven any theoretical guarantees for discrete optimization problems, REMBO appears to effectively exploit the low effective dimensionality of at least this particular optimization problem.

\begin{figure}[tb]
\begin{center}
  \includegraphics[scale=0.41]{figures/lpsolve.png}
  \includegraphics[scale=0.41]{figures/lpsolve_interleave.png}
  \caption{Performance of various methods for configuration of \texttt{lpsolve}; we show the optimality gap \texttt{lpsolve} achieved with the configurations found by the various methods (lower is better). Left: a single run of each method; Right: performance with $k=4$ interleaved runs.\label{fig:lpsolve}}
\end{center}
\end{figure}

Figure \ref{fig:lpsolve} (left) compares BO, REMBO, and the baseline random search against 
ParamILS \cite{ParamILS-JAIR} 
%(which was used for all configuration experiments by~\citeA{Hutter:2010}), 
and SMAC \cite{Hutter:2011}. 
ParamILS and SMAC were specifically designed for the configuration of algorithms with many discrete parameters and define the current state of the art for this problem. Nevertheless, here SMAC and our vanilla REMBO method performed best. Based on a Mann-Whitney U test with Bonferroni multiple-test correction, they both yielded statistically significantly better results than both Random and standard BO; no other performance differences were significant.
The figure only shows REMBO with $d=5$ to avoid clutter, but we did not optimize this parameter; the only other value we tried ($d=3$) resulted in indistinguishable . 

As in the synthetic experiment, REMBO's performance could be further improved by using multiple interleaved runs.
However, as shown by~\citeA{HutHooLey12-ParallelAC}, multiple independent runs can also improve the performance of SMAC and especially ParamILS. 
Thus, to be fair, we re-evaluated all approaches using interleaved runs. Figure \ref{fig:lpsolve} (right) shows that ParamILS and REMBO benefitted most from interleaving $k=4$ runs. However, the statistical test results did not change, still showing that SMAC and REMBO outperformed Random and BO, with no other significant performance differences.



==> embedding_arxiv/linearProg_old.tex <==
State-of-the-art algorithms for solving hard computational problems tend to parameterize several design choices in order to allow a customization of the algorithm to new problem domains. Automated methods for algorithm configuration have recently demonstrated that substantial performance gains of state-of-the-art algorithms can be achieved in a fully automated fashion~\cite{Mockus:1999,Hutter:2010,Bergstra:2011,Wang:2011}. These successes have led to a paradigm shift in algorithm development towards the active design of highly parameterized code followed by automated procedures to best instantiate this code for a given problem domain~\cite{Hoos:2012:PO:2076450.2076469,Bergstra:model_search}.

It has long been suspected that these algorithm configuration problems have low dimensionality~\cite{Hutter:2009}. Here, we demonstrate that REMBO can exploit this low dimensionality even in the discrete spaces typically encountered in algorithm configuration. 
We use a configuration problem obtained from \citeA{Hutter:2010}, aiming to configure the 40 binary and 7 categorical parameters of \text{lpsolve}\footnote{http://lpsolve.sourceforge.net/}, a popular mixed integer linear programming solver that has been downloaded over 40\,000 times in the last year.
The objective is to minimize the optimality gap \texttt{lpsolve} can obtain in a fixed time limit of five seconds for a mixed integer programming (MIP) encoding of a wildlife corridor problem from computational sustainability~\cite{ghs08:connection}.
Algorithm configuration usually aims to improve performance for a representative set of problem instances, and effective methods need to solve two orthogonal problems: searching the parameter space effectively and deciding how many instances to use in each evaluation (to trade off computational overhead and over-fitting). Our contribution is for the first of these problems; to focus on how effectively different methods search the parameter space, we only consider configuration on a single problem instance.

Due to the discrete nature of this optimization problem, we could only apply REMBO using the high-dimensional kernel for categorical variables $k^D_{\lambda}(\vy^{(1)}, \vy^{(2)})$ described in Section \ref{sec:choice_of_kernel}. While we have not proven any theoretical guarantees for discrete optimization problems, REMBO appears to effectively exploit the low effective dimensionality of this particular optimization problem.

\begin{figure}[tb]
\begin{center}
  \includegraphics[scale=0.35]{figures/lpsolve.png}\\
  \includegraphics[scale=0.35]{figures/lpsolve_interleave.png}
  \caption{Performance of various methods for configuration of \texttt{lpsolve}; we show the optimality gap \texttt{lpsolve} achieved with the configurations found by the various methods (lower is better). Top: a single run of each method; Bottom: performance with $k=4$ interleaved runs.}
\end{center}
\vspace*{-2mm}
\label{fig:lpsolve} 
\end{figure}


Figure \ref{fig:lpsolve} (top) compares BO, REMBO, and the baseline random search against the configuration procedures ParamILS (which was used for all configuration experiments in~\cite{Hutter:2010}),
%ParamILS~\cite{ParamILS-JAIR} (which was used for all configuration experiments in~\cite{Hutter:2010}), 
and SMAC \cite{Hutter:2011}. ParamILS and SMAC have been specifically designed for the configuration of algorithms with many parameters and define the current state of the art for this problem. As the figure shows, they indeed outperformed both BO and random search by a comfortable margin. However, remarkably, our vanilla REMBO method performed even slightly better. While the figure only shows REMBO with $d=5$ to avoid clutter, we by no means optimized this parameter; the only other value we tried was $d=3$, which resulted in indistinguishable performance. 

As in the synthetic experiment, REMBO's performance could be further improved by using multiple interleaved runs.
However, it is known that multiple independent runs can also improve the performance of the other procedures, especially ParamILS~\cite{HutHooLey12-ParallelAC}. Thus, to be fair, we re-evaluated all approaches using interleaved runs. Figure \ref{fig:lpsolve} (bottom) shows that when using $k=4$ interleaved runs of $500$ evaluations each, REMBO and ParamILS performed best, with a slight advantage for REMBO early on in the search.


%\note{FH: Ziyu, to get confidence in the wider applicability of this result, I'd like to do some additional experiments on more instances. Let's talk about them...}






==> embedding_arxiv/millionDimensions.tex <==
%!TEX root = embedding.tex

%In this section, we study REMBO's invariance properties using synthetic data, empirically evaluate strategies for increasing its success probability,
%and, most importantly, add empirical evidence to our theoretical finding from Section \ref{sec:rembo} that REMBO's performance is independent of the extrinsic dimensionality $D$
%when using the low-dimensional kernel $k_{\ell}^d(\vy^1, \vy^2)$.
%We show that when using that kernel, REMBO has no problem scaling up to as many as $1$ billion dimensions.

\begin{figure*}[t!]
\centering
  \includegraphics[scale=0.5]{figures/branin_dis_25.png}
  \includegraphics[scale=0.5]{figures/branin_dis_rot.png}
  \includegraphics[scale=0.5]{figures/branin_dis_1b.png}
  \caption{Comparison of random search (RANDOM), Bayesian optimization (BO),
  method by~\protect\citeA{Chen:2012} (HD BO), and REMBO.
Left: $D=25$ extrinsic dimensions; Right: $D=25$, with a rotated objective function; Bottom: $D=10^9$ extrinsic dimensions. We plot means and $1/4$ standard deviation confidence intervals of the optimality gap across 50 trials.}
  \label{fig:standard}
\end{figure*}

The experiments in this section employ a standard $d_e=2$-dimensional benchmark function for Bayesian optimization, embedded in a $D$-dimensional space. That is, we add $D-2$ additional dimensions which do not affect the function at all.
More precisely, the function whose optimum we seek is $f(\vx_{1:D}) = g(x_i,x_j)$, where $g$ is the Branin function
\begin{eqnarray*}
g(x_1, x_2) 
= (x_2- \frac{5.1}{4\pi^2}x_1^2 + \frac{5}{\pi}x_1 - 6)^2 + 
10(1-\frac{1}{8\pi})\cos(x_1) + 10
\end{eqnarray*}
and where $i$ and $j$ are selected once using a random permutation.
To measure the performance of each optimization method, we used the \emph{optimality gap}: the difference of the best function value it found and the optimal function value.   

\begin{table}[h]
\small
\begin{center}
\begin{tabular}{ l |  c  c  c}
\hline
$k$ & $d=2$ & $d=4$ & $d=6$ \\
\hline
  10& 0.0022 $\pm$ 0.0035 & 0.1553 $\pm$ 0.1601 & 0.4865 $\pm$  0.4769 \\
  5 & 0.0004 $\pm$ 0.0011 & 0.0908 $\pm$ 0.1252 & 0.2586 $\pm$ 0.3702 \\
  4 & 0.0001 $\pm$ 0.0003 & 0.0654 $\pm$ 0.0877 & 0.3379 $\pm$ 0.3170 \\
  2 & 0.1514 $\pm$ 0.9154 & 0.0309 $\pm$ 0.0687 & 0.1643 $\pm$ 0.1877 \\
  1 & 0.7406 $\pm$ 1.8996 & 0.0143 $\pm$ 0.0406 & 0.1137 $\pm$ 0.1202 \\
\end{tabular}
\end{center}
\caption{Optimality gap for $d_e=2$-dimensional Branin function embedded in $D=25$ dimensions, for
REMBO variants using a total of $500$ function evaluations. The variants differed in the internal dimensionality $d$ and in the number of interleaved runs $k$ (each such run was only allowed $500/k$ function evaluations).
%We initialized all methods to the same random point and 
We show mean and standard deviations of the optimality gap achieved after 500 function evaluations. 
\label{tab:rembo_variants_results}}
\end{table}

We evaluate REMBO using a fixed budget of $500$ function
evaluations that is spread across multiple interleaved runs ---
for example, when using $k = 4$ interleaved REMBO runs,
each of them was only allowed $125$ function evaluations. 
We study the choices of $k$ and $d$ by considering several combinations of these values.
The results in Table \ref{tab:rembo_variants_results} demonstrate that interleaved runs helped improve REMBO's performance.
We note that in 13/50 REMBO runs, the global optimum was indeed not contained in the box $\mathcal{Y}$ REMBO searched with $d=2$; this is the reason for the poor mean performance of REMBO with $d=2$ and $k=1$.
However, the remaining $37$ runs performed very well, and REMBO thus performed well when using multiple interleaved runs: with a failure rate of 13/50=0.26 per independent run, the failure rate using $k=4$ interleaved runs is only $0.26^4\approx 0.005$. One could easily achieve an arbitrarily small failure rate by using many independent parallel runs. 
Using a larger $d$ is also effective in increasing the probability of the optimizer falling into REMBO's box $\mathcal{Y}$ but at the same time slows down REMBO's convergence (such that interleaving several short runs loses its effectiveness). 
 
Next, we compared REMBO to standard Bayesian optimization (BO) and to random search, for an extrinsic dimensionality of $D=25$. 
Standard BO is well known to perform well in low dimensions, but to degrade above a tipping point of about 15-20 dimensions. Our results for $D=25$ (see Figure \ref{fig:standard}, left) confirm that BO performed rather poorly just above this critical dimensionality (merely tying with random search). 
REMBO, on the other hand, still performed very well in 25 dimensions.

One important advantage of REMBO is that --- in contrast to the approach of \citeA{Chen:2012} --- it does not require the effective dimension to be coordinate aligned. To demonstrate this fact empirically, we rotated the embedded Branin function by an orthogonal rotation matrix $\vR \in \mathbb{R}^{D\times D}$. That is, we replaced $f(\vx)$ by $f(\vR \vx)$.
Figure~\ref{fig:standard} (middle) shows that REMBO's performance is not affected by this rotation. 

Finally, since REMBO is independent of the extrinsic dimensionality $D$ as long as the intrinsic dimensionality $d_e$ is small, it performed just as well in $D=1\,000\,000\,000$ dimensions (see Figure \ref{fig:standard}, right). 
To the best of our knowledge, the only other existing method that can be run in such high dimensionality is random search.

For reference, we also evaluated the method of \citeA{Chen:2012} for these functions, confirming that it does not handle rotation gracefully: 
while it performed best in the non-rotated case for $D=25$, it performed worst in the rotated case. It could not be used efficiently for more than $D=1,000$.
Based on a Mann-Whitney U test with Bonferroni multiple-test correction, all performance differences were statistically significant, except Random vs.\ standard BO.
% \textcolor{red} {
Finally, comparing REMBO to the method of \citeA{Chen:2012}, we also note that REMBO is much simpler to implement and that its results are very reliable (with interleaved runs).
% }


% \textcolor{magenta} {
\subsection{Synthetic Discrete Experiment}
In this section, we test the high-dimensional kernel with a synthetic experiment. Specifically, we again optimize the Branin function, but restrict its domain to $225$ discrete points on a regular grid.
As above, we added $23$ additional irrelevant dimensions to make the problem 25-dimensional in total. 
% }

% \textcolor{magenta} {
We used a small fixed budget of $100$ function evaluations for all algorithms involved as the problem would require no more than $225$ evaluations to be solved completely. We used $k=4$ interleaved runs for REMBO.
We again compare REMBO to random search and standard BO. For REMBO, we use the high-dimensional kernel to handle the discrete nature of the problem.
The result of the comparison is summarized in Figure~\ref{fig:disbran}.
Standard BO again suffered from the high extrinsic dimensionality
and performed slightly worse than random search. REMBO, on the other hand, performed well in this setting.
% }
\begin{figure*}[t!]
\centering
  \includegraphics[scale=0.5]{figures/ac6.png}
  \caption{Comparison of random search (RANDOM), Bayesian optimization (BO), and REMBO. $D=25$ extrinsic dimensions. We plot means and $1/4$ standard deviation confidence intervals of the optimality gap across 50 trials.}
  \label{fig:disbran}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLD ARXIV VERSION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we add empirical evidence to our theoretical finding from Section \ref{sec:rembo} that REMBO's performance is independent of the extrinsic dimensionality $D$
% when using the low-dimensional kernel $k_{\ell}^d(\vy^1, \vy^2)$ from Definition \ref{def:sekernel}.
% Specifically, using synthetic data, we show that when using that kernel REMBO has no problem scaling up to as many as $1$ billion dimensions. We also study REMBO's invariance properties and empirically evaluate our two strategies for increasing its success probability.

% The experiments in this section employ a standard $d_e=2$-dimensional benchmark function for Bayesian optimization, embedded in a $D$-dimensional space. That is, we add $D-2$ additional dimensions which do not affect the function at all.
% More precisely, the function whose optimum we seek is $f(\vx_{1:D}) = b(x_i,x_j)$, where $b$ is the Branin function
% \cite[see][for its exact formula]{Lizotte:2008_PhD},
% \note{FH: just define the function here instead of referring to elsewhere} and where dimensions $i$ and $j$ are selected once using a random permutation of $1,\dots,D$.
% % $1:D$.
% %
% To measure the performance of each optimization method, we used the \emph{optimality gap}: the difference of the best function value it found and the optimal function value.   

% %; $i$ and $j$ stay constant during the run of each algorithm.

% \begin{table}[t]
% \scriptsize
% \begin{center}
% \begin{tabular}{ l |  c  c  c}
% \hline
% $k$ & $d=2$ & $d=4$ & $d=6$ \\
% \hline
%   10& 0.0022 $\pm$ 0.0035 & 0.1553 $\pm$ 0.1601 & 0.4865 $\pm$  0.4769 \\
%   5 & 0.0004 $\pm$ 0.0011 & 0.0908 $\pm$ 0.1252 & 0.2586 $\pm$ 0.3702 \\
%   4 & 0.0001 $\pm$ 0.0003 & 0.0654 $\pm$ 0.0877 & 0.3379 $\pm$ 0.3170 \\
%   2 & 0.1514 $\pm$ 0.9154 & 0.0309 $\pm$ 0.0687 & 0.1643 $\pm$ 0.1877 \\
%   1 & 0.7406 $\pm$ 1.8996 & 0.0143 $\pm$ 0.0406 & 0.1137 $\pm$ 0.1202 \\
% \end{tabular}
% \end{center}
% \caption{Optimality gap for $d_e=2$-dimensional Branin function embedded in $D=25$ dimensions, for
% REMBO variants using a total of $500$ function evaluations. The variants differed in the internal dimensionality $d$ and in the number of interleaved runs $k$ (each such run was only allowed $500/k$ function evaluations).
% %We initialized all methods to the same random point and 
% We show mean and standard deviations of the optimality gap achieved after 500 function evaluations. 
% \label{tab:rembo_variants_results}}
% \label{fig:braninresult}
% \end{table}

% \begin{figure*}[tb]
% \centering
%   \includegraphics[scale=0.3]{figures/branin_dis_25D.png}
%   \includegraphics[scale=0.3]{figures/branin_dis_1bil.png}
%   \includegraphics[scale=0.3]{figures/branin_dis_rotation.png}
%   \caption{Comparison of random search (RANDOM), standard Bayesian optimization (BO), and REMBO.
% Left: $D=25$ extrinsic dimensions; Middle: $D=1\,000\,000\,000$ extrinsic dimensions; Right: $D=25$, with a rotated objective function. For each method, we plot means and $1/4$ standard deviation confidence intervals of the optimality gap across 50 trials.}
%   \label{fig:standard}
%   \vspace{-1.0em}
% \end{figure*}


% \note{FH: for me: this paragraph could be improved in structure a bit.}
% We first study the effectiveness of the two techniques for increasing REMBO's success probability that we proposed in Section \ref{sec:increasing_rembo_success}.
% %that the global optimizer lies in the box $\mathcal{Y}$ REMBO searches 
% To empirically study the effectiveness of using internal dimensionalities $d>d_e$, and of interleaving multiple independent runs, $k$, we ran REMBO with
% all combinations of three different values of $d$ and $k$.
% The results in Table \ref{tab:rembo_variants_results} demonstrate that both techniques helped improve REMBO's performance, with interleaved runs being the more effective strategy.
% %, a potential problem is that the true optimizer may not be contained in the box $\mathcal{Y}$ REMBO searches. 
% %In that section, we also proposed two techniques for alleviating this problem: 
% We note that in 13/50 REMBO runs, the global optimum was indeed not contained in the box $\mathcal{Y}$ that REMBO searched with $d=2$; this is the reason for the poor mean performance of REMBO with $d=2$ and $k=1$.
% %
% However, the remaining $37$ runs performed very well, and REMBO thus performed well when using multiple interleaved runs: with a failure rate of 13/50=0.26 per independent run, the failure rate using $k=4$ interleaved runs is only $0.26^4\approx 0.005$. One could easily achieve an arbitrarily small failure rate by using many independent parallel runs. Here we evaluated all REMBO versions using a fixed budget of $500$ function evaluations that is spread across multiple interleaved runs --- for example, when using $k=4$ interleaved REMBO runs, each of them was only allowed 125 function evaluations. 
% %
% The results show that performing multiple independent runs nevertheless substantially improved REMBO's performance. Using a larger $d$ was also effective in increasing the probability of the optimizer falling into REMBO's box $\mathcal{Y}$ but at the same time slowed down REMBO's convergence (such that interleaving several short runs lost its effectiveness). We conclude that using several interleaved runs of REMBO with small $d \ge d_e$ performs best.
 
% %This was not a problem for REMBO when using $d=2$ since it converged quickly in this low-dimensional space. Of course, even for this quick convergence there comes a point where we are interleaving too many independent runs (\eg{}, $k=10$) 

% %However, using a higher-dimensional embedding ($d=4$ or $d=6$) slowed down convergence to the point where interleaving runs did not improve performance anymore.

% %\hide{For example, with $5$ consecutive runs and $d=d_e=2$, we found that $\mathcal{Y}$ always captured the optimizer in our experiments. %In following this strategy, we took the best of the $5$ runs. When using a single run but $d=4$, we observed $2$ failures in $60$ runs. For these failures, REMBO converged to rather poor solutions, but in order to keep the comparison fair, these $2$ cases were included in the averages shown in the table and plots.}

% \note{Chen et al is not discussed here -- maybe use the version from IJCAI to start with?}
% Next, we compared REMBO to standard Bayesian optimization (BO) and to random search, for an extrinsic dimensionality of $D=25$.
% %This plot shows the large margin by which REMBO outperforms both standard BO and random search in 25 dimensions.  
% Standard BO is well known to perform well in low dimensions, but to degrade above a tipping point of about 15-20 dimensions. Our results for $D=25$ (see Figure \ref{fig:standard}, left) confirm that BO performed quite poorly just above this critical dimensionality (merely tying with random search). 
% REMBO, on the other hand, still performed very well in 25 dimensions.


% %All REMBO variants, on the other hand, still performed very well in 25 dimensions. In order to evaluate our first technique for increasing REMBO's success probability (see Section \ref{sec:increasing_rembo_success}), we chose three different values for REMBO's intrinsic dimensionality $d$. As expected, the ``true'' value of $d=d_e=2$ yielded the fastest search initially, but not all REMBO runs  could find the optimum. Higher values of $d$ yielded slower convergence but were able to find better solutions in the end. 


% %Next, we evaluated our second strategy for increasing REMBO's success rate: performing multiple independent parallel runs and using the result of the best. This technique can in principle improve the performance of all algorithms (including random search and standard BO), but since REMBO has much larger variance, it benefits most from this technique. Figure \ref{fig:standard} (middle) shows the results for performing 4 independent parallel runs of each technique; comparing to \ref{fig:standard} (top), we note that REMBO's performance was improved most by this technique.

% % in our experiments. That is, if we choose $d=4$, then the 4-dimensional vector $\vy$ is projected to a vector $\vx=\vA\vy$ in $D$ dimensions. We then evaluate the function $f(x_1,x_2,\vx_{3:D})$, which simply returns the Branin value $f(x_1,x_2)$ because there are only two relevant dimensions. The advantage of REMBO over other methods is very clear here. Since REMBO optimizes in $d$ instead of $D$, it is irrelevant how high $D$ is. The same is not true for other methods. We could not run standard Bayesian optimization in a billion dimensions in a reasonable time.

% Since REMBO is independent of the extrinsic dimensionality $D$ as long as the intrinsic dimensionality $d_e$ is small, it performed just as well in $D=1\,000\,000\,000$ dimensions (see Figure \ref{fig:standard}, middle). 
% To the best of our knowledge, the only other existing method that can be run in such high dimensionality is random search.

% Finally, one important advantage of REMBO is that --- in contrast to the approach of \citeA{Chen:2012} --- it does not require the effective dimension to be coordinate aligned. To demonstrate this fact empirically, we rotated the embedded Branin function by an orthogonal rotation matrix $\vR \in \mathbb{R}^{D\times D}$. That is, we replaced $f(\vx)$ by $f(\vR \vx)$.
% Figure~\ref{fig:standard} (right) shows that REMBO's performance is not affected by this rotation. 
% %
% %The bottom plot makes the case that REMBO's performance does not deteriorate as the extrinsic dimensionality becomes extremely large; provided that the intrinsic dimensionality of the problem is low.




% %This is in agreement with the theory.  

%  %
% % 
% %First, we empirically studied the percentage of random embeddings under which at least one true optimizer is contained in $\mathcal{B} = [0, 1]^d$. Table \ref{table:perc} shows that these empirical percentages are around $0.6$ for both functions.
% %Next, we studied REMBO performance under the condition that one optimizer indeed falls into $\mathcal{B}$. As Figure \ref{fig:standard} shows that REMBO run on the 1\,000\,000-dimensional functions of low effective dimensionality was as effective as BO on the original functions. 
% %%
% %
% %
% %In practice, we do not know whether a function's optimizer falls into $\mathcal{B}$ for a given embedding. There are multiple possible ways to guard against this problem. The first is to simply run REMBO multiple times with different independently drawn random embeddings. 
% %%
% %Observe that for our two example problems repeating REMBO $5$ times each with $100$ iterations could locate the optimizer with failure probability of roughly $(1-0.6)^5 \approx 0.01$ in 1\,000\,000 dimensions. 
% %In contrast, pure BO failed to find the optimum within $500$ iterations when run on the original functions embedded in as little as 20 dimensions. Further, running pure BO at all quickly becomes infeasible in high dimensions whereas our approach scales up to arbitrary high dimensions as long as the effective dimensionality is relatively low. 
% %%\note{FH: Is the success probability independent of the extrinsic dimension?}
% %
% %The second possibility to increase the probability of the optimizer falling into the bounds is to increase the dimensionality $d$ REMBO operates on. Figure \ref{fig:standard}~(left) shows results for $d=4$, in this case not asserting that the optimizer falls into $\mathcal{B}$. REMBO is somewhat slower due to this increase in dimension but still manages to locate the optimum after $400$ iterations. Empirically, when $d=4$ and $\mathcal{B} = [0, 1]^d \times \sqrt d$, the probability of at least one optimizer falling into $\mathcal{B}$ was approximately $0.99$. 
% %%\note{FH: Can we argue that that probability would be approximately $(1-0.6)^{\binom{4}{2}}$?}
% %Overall, these experiments show that we can effectively optimize extremely high-dimensional functions with effective low dimensionality, even if the low dimension is not axis aligned.

% % For both functions the proposed approach works as well as BO on the original problem given that an optimizer is contained in the lower dimensional bounding box $\mathcal{B}$. Both methods approach the true global optimum. Pure Bayesian optimization in high dimensions, however, did not approach the global optimum. By increasing $d$ from $2$ to $4$, we see that the failure probability decreases dramatically and REMBO approaches the optimizer consistently. Finally, the plot showes that REMBO can handle effective dimensions that are not coordinate-aligned as it works effectively on rotated functions.

% %\note{FH: I was somewhat concerned by the remark: `We attribute this to our choices of hyper-parameters for the GP.' Did you choose them manually?}

% \hide{
% %FH: I found this description somewhat repetitive - please feel free to undo some of my changes (that's why I left the original sources here).
% For the Branin function, we conducted the following experiments. First to compare to the best possible scenario, we do Bayesian optimization directly on the Branin function. Next, to study the effect of extrinsic dimensionality on the proposed approach, we embed the Branin function in a one million dimensional space and run the proposed approach. As discussed in the previous section, we know that the true optimizer does not always fall into the bound $\mathcal{B}$ in the lower dimensional space. To illustrate the efficiency of our method we ensured that at least one optimizer falls into $\mathcal{B}$ by repeatedly drawing $\vA$. Here $\mathcal{B}$ is chosen to be $[0, 1]^d$. 

% For the third experiment, we choose our embedding dimension $d$ to be $4$ which is higher than the effective dimension $d_e = 2$. We show that by doing this, the failure probability decreases dramatically. Unlike in the previous experiment, we do not try to ensure that an optimizer falls into $\mathcal{B}$. To further lower the probability of not including an optimizer, we set the bound to be $[0, 1]^d \times \sqrt d$. In doing so we lowered the probability of failure to $0.01$.

% The fourth experiment shows that our approach is still valid when the effective dimensions are not coordinate-aligned. The embedded Branin function is rotated by an orthogonal rotation matrix $R \in \mathbb{R}^{D\times D}$. As in the last $2$ experiments, we set $D$ to be one million and ensure that one optimizer falls into $\mathcal{B}$ where $\mathcal{B} = [0, 1]^d$. Finally, we embed the Branin function in a $20$ dimensional space and try Bayesian optimization on this high dimensional space. 

% All of the above experiments are repeated $20$ times each with $500$ iterations. Figure \ref{fig:standard}~(left) presents the result by summarizing the mean and $\frac{1}{5}$ of the standard deviation of $G_t$ across different runs. Notice that when an optimizer is contained in $\mathcal{B}$, REMBO is comparable to the BO when $d = 2$ as they both locate the maximum well within $100$ iterations. This is significant as it demonstrates that REMBO is not affected by the extrinsic dimensionality which in this case is one million. 
% In Table 1 we summarize the empirical percentage of times where the true optimizer is contained in $\mathcal{B} = [0, 1]^d$. Although we can not guarantee that the true optimizer is contained in $\mathcal{B}$, we argue that REMBO is still preferable over BO when the dimensionality is high. Observe that BO in $20$ dimensions could not find the maximum within $500$ iterations while by repeating REMBO $5$ times each with $100$ iterations, we can locate the optimizer with failure probability approximately equal to $(1-0.5951)^5 = 0.0109$. Further, we must remember that BO would become infeasible in high dimensions whereas our approach would scale up to arbitrary high dimensions as long as the effective dimensionality is relatively low. Figure \ref{fig:standard}~(left) also shows that despite the fact that we do not check whether the optimizer falls into $\mathcal{B}$ when $d=4$, REMBO still manages to locate the optimum after $400$ iterations. The experimental results show that when $d=4$ and $\mathcal{B} = [0, 
% 1]^d \times \sqrt d$, the probability of having at least one optimizer in $\mathcal{B}$ is approximately $0.99$. Whereas the approach of Chen et al \cite{Chen:2012} requires the effective dimension to be coordinate aligned, REMBO does not.  

% For the Hartmann3 function, we compared REMBO with BO in the original and high dimensional space. All of the experiments are repeated $20$ times each with $200$ iterations. Figure \ref{fig:standard}~(right) summarizes the result by plotting the mean and $\frac{1}{5}$ of the standard deviation $G_t$. The results on the Hartmann3 confirms the findings from the Branin function. It is interesting to note, however, REMBO in this case converges faster than BO in the original space. We attribute this to our choices of hyper-parameters for the GP.
% }



==> embedding_arxiv/mydef.tex <==
%dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi

\usepackage{amsmath,amsthm,amssymb}
%\usepackage{amsfonts}

\usepackage{color}
\definecolor{Blue}{rgb}{0.9,0.3,0.3}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}

%% a trick that makes the title take up less space for many style files (but not article)
%\addtolength{\titlebox}{-1.8cm}

%% densify spacing in bibliographies
\newcommand{\bibfix}{%    PUT \bibfix in file.bbl after first line
    \setlength{\parsep}{\parskip}%
    \setlength{\itemsep}{0cm}%
    \setlength{\topsep}{\parskip}%
    \setlength{\parskip}{0cm}%
    \setlength{\partopsep}{0cm}%
    \setlength{\listparindent}{\parindent}%
    \setlength{\labelwidth}{10pt}%
    \setlength{\labelsep}{0pt}%
    \setlength{\leftskip}{0pt}%
    \setlength{\leftmargin}{0pt}%
}

%% change margins
%\setlength{\textwidth}{7in}
%\setlength{\textheight}{8.75in}
%\setlength{\oddsidemargin}{-0.25in}
%\setlength{\evensidemargin}{-0.25in}
%\setlength{\headsep}{10pt}

%Use changebar.sty  to track changes.

%Saving space: see
%   http://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html

%Page layout info:
%   http://amath.colorado\edu/documentation/LaTeX/reference/layout.html


%%%%%%%%%% Code listings



%Latex
%\documentstyle[fleqn,psfig,epsfig]{article}
%\documentstyle[psfig]{article}
%\setlength{\textwidth}{6.5in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\textheight}{8.5in}
%\setlength{\headheight}{0in}
%\setlength{\headsep}{0in}
%\setlength{\parindent}{0in} % block style
%\setlength{\parskip}{0.3cm}

\newtheorem{example}{Example}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}
\newenvironment{myproof}{{\bf Proof}}{}

%http://www.maths.tcd.ie/~dwilkins/LaTeXPrimer/Theorems.html
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

% make qed symbol a solid square
%\renewcommand{\qed}{\mbox{$\hrulefill \blacksquare $}}

%http://everything2.com/title/tombstone
%\renewcommand{\qed}{\hfill \nobreak \ifvmode \relax \else
%    \ifdim\lastskip<1.5em \hskip-\lastskip
%    \hskip1.5em plus0em minus0.5em \fi \nobreak
%    \vrule height0.4em width0.4em depth0.25em\fi}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
%\newcommand{\half}{\frac{1}{2}}
\newcommand{\half}{\frac{1}{2}}
%\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\defeq}{:=}
%\newcommand{\real}{{\rm I\hspace{-0.2em}R}}
\newcommand{\real}{\mathbb{R}}
%\newcommand{\indep}{\perp}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

%\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\trans}[1]{{#1}^{T}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\st}{\; \mathrm{s.t.} \;}
%\newcommand{\det}{\mathrm{det}}
\newcommand{\size}{\mathrm{size}}
\newcommand{\trace}{\mathrm{trace}}

%\newcommand{\do}{\mathrm{do}}
\newcommand{\pemp}{p_\mathrm{emp}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\bel}{\mathrm{bel}}
\newcommand{\dsep}{\mathrm{dsep}}
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mathrm{range}}
\newcommand{\myspan}{\mathrm{span}}
\newcommand{\nullspace}{\mathrm{nullspace}}
\newcommand{\adj}{\mathrm{adj}}
\newcommand{\pval}{\mathrm{pvalue}}
\newcommand{\NLL}{\mathrm{NLL}}


\newcommand{\betadist}{\mathrm{Beta}}
\newcommand{\Betadist}{\mathrm{Beta}}
\newcommand{\bernoulli}{\mathrm{Ber}}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Binom}{\mathrm{Bin}}
\newcommand{\NegBinom}{\mathrm{NegBinom}}
\newcommand{\binomdist}{\mathrm{Bin}}
\newcommand{\cauchy}{\mathrm{Cauchy}}
\newcommand{\DE}{\mathrm{DE}}
\newcommand{\DP}{\mathrm{DP}}
\newcommand{\Dir}{\mathrm{Dir}}
%\newcommand{\discrete}{\mathrm{Discrete}}
\newcommand{\discrete}{\mathrm{Cat}}
\newcommand{\Discrete}{\discrete}
\newcommand{\expdist}{\mathrm{Exp}}
\newcommand{\expon}{\mathrm{Expon}}
\newcommand{\gammadist}{\mathrm{Ga}}
\newcommand{\Ga}{\mathrm{Ga}}
\newcommand{\GP}{\mathrm{GP}}
\newcommand{\GEM}{\mathrm{GEM}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\erlang}{\mathrm{Erlang}}
%\newcommand{\IG}{\mathrm{InvGam}}
\newcommand{\IG}{\mathrm{IG}}
\newcommand{\IGauss}{\mathrm{InvGauss}}
\newcommand{\IW}{\mathrm{IW}}
\newcommand{\Laplace}{\mathrm{Lap}}
\newcommand{\logisticdist}{\mathrm{Logistic}}
\newcommand{\Mu}{\mathrm{Mu}}
\newcommand{\Multi}{\mathrm{Mu}}
%\newcommand{\Multin}{\mathrm{Mun}}
%\newcommand{\Mun}{\mathrm{Mun}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mathrm{NIG}}
\newcommand{\GIG}{\mathrm{NIG}}
\newcommand{\NIW}{\mathrm{NIW}}
\newcommand{\GIW}{\mathrm{NIW}}
%\newcommand{\MVNIW}{\mathrm{MVNIW}}
\newcommand{\MVNIW}{\mathrm{NIW}}
\newcommand{\NW}{\mathrm{NWI}}
\newcommand{\NWI}{\mathrm{NWI}}
%\newcommand{\MVNIG}{\mathrm{MVNIG}}
\newcommand{\MVNIG}{\mathrm{NIG}}
\newcommand{\NGdist}{\mathrm{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mathrm{Wi}}
\newcommand{\Wi}{\mathrm{Wi}}
\newcommand{\unif}{\mathrm{U}}
\newcommand{\etr}{\mathrm{etr}}


%\newcommand{\dim}{\mathrm{dim}}
\newcommand{\mse}{\mathrm{mse}}
\newcommand{\pon}{\rho}
\newcommand{\lse}{\mathrm{lse}}
\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mathrm{soft}}
\newcommand{\cond}{\mathrm{cond}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mathrm{wp}}

\newcommand{\KLpq}[2]{\mathbb{KL}\left({#1}||{#2}\right)}
\newcommand{\KL}{\mathbb{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entrop}{\mathbb{H}}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}

%\newcommand{\myvec}[1]{\mathbf{#1}}
%\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\myvec}[1]{\mathbf{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}
%\newcommand{\ind}[1]{[#1]}


\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}

\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
%\newcommand{\vEta}{\myvecsym{\Eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vmut}{\myvecsym{\tilde{\mu}}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vPi}{\myvecsym{\Pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vthetat}{\myvecsym{\tilde{\theta}}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vSigmat}{\myvecsym{\tilde{\Sigma}}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mathrm{const}}
\newcommand{\sigmoid}{\mathrm{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwt}{\myvec{\tilde{w}}}
\newcommand{\vWt}{\myvec{\tilde{W}}}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vra}{\myvec{r}_a}
\newcommand{\vwa}{\myvec{w}_a}
\newcommand{\vXa}{\myvec{X}_a}


\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vMt}{\myvec{\tilde{M}}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}
\newcommand{\vZt}{\myvec{\tilde{Z}}}
\newcommand{\vzt}{\myvec{\tilde{z}}}

\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mathrm{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\rbar}{\overline{r}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vAbar}{\overline{\vA}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\wbar}{\overline{w}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}
\newcommand{\mubar}{\overline{\mu}}
\newcommand{\phibar}{\overline{\phi}}


\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}



%\newcommand{\sss}{s^2}
%\newcommand{\vvv}{v}
\newcommand{\RSS}{\mathrm{RSS}}
\newcommand{\mydof}{\mathrm{dof}}



\newcommand{\vvec}{\mathrm{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mathrm{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expectQ}[2]{\mathbb{E}_{{#2}} \left[ {#1} \right]}
\newcommand{\Var}{\mathrm{Var}}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mathrm{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mathrm{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mathrm{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mathrm{cov}\left[{#1}\right]}
\newcommand{\corr}[1]{\mathrm{corr}\left[{#1}\right]}
\newcommand{\mode}[1]{\mathrm{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mathrm{median}\left[{#1}\right]}




\newcommand{\sech}{\mathrm{sech}}
%\newcommand{\cosh}{\mathrm{cosh}}
\newcommand{\kurt}{\mathrm{kurt}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\myskew}{\mathrm{skew}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\blkdiag}{\mathrm{blkdiag}}
\newcommand{\bias}{\mathrm{bias}}
%\newcommand{\dim}{\mathrm{dim}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}



%\newcommand{\NN}{N}
%\newcommand{\NC}{N_C}
%\newcommand{\ND}{N_D}
%\newcommand{\NX}{N_X}
%\newcommand{\NXi}{N_{X_i}}
%\newcommand{\NY}{N_Y}
%\newcommand{\nx}{n_x}
%\newcommand{\ny}{n_y}
%\newcommand{\nv}{n_v}
%\newcommand{\nk}{n_k}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}



\newcommand{\kernelfn}{\kappa}

\newcommand{\Nsamples}{S}
\newcommand{\Ndata}{N}
\newcommand{\Ntrain}{N_{\mathrm{train}}}
\newcommand{\Ntest}{N_{\mathrm{test}}}
\newcommand{\Ndim}{D}
\newcommand{\Ndimx}{D_x}
\newcommand{\Ndimy}{D_y}
\newcommand{\Nhidden}{H}
\newcommand{\Noutdim}{D_y}
\newcommand{\Nlowdim}{L}
\newcommand{\Ndimlow}{L}
\newcommand{\Nstates}{K}
\newcommand{\Nfolds}{K}
\newcommand{\Npastates}{L}
\newcommand{\Nclasses}{C}
\newcommand{\Nclusters}{K}
\newcommand{\NclustersC}{C}
\newcommand{\Ntime}{T}
\newcommand{\Ntimes}{T}
\newcommand{\Niter}{T}
\newcommand{\Nnodes}{D}

\newcommand{\assign}{\leftarrow}



%\newcommand{\xdi}{x_{di}}
%\newcommand{\xji}{x_{ji}}
%\newcommand{\yi}{y_i}



\newcommand{\ki}{i}
\newcommand{\kj}{j}
\newcommand{\kk}{k}
\newcommand{\kC}{C}
\newcommand{\kc}{c}

\newcommand{\supp}{\mathrm{supp}}
\newcommand{\query}{\calQ}
\newcommand{\vis}{\calE}
\newcommand{\nuisance}{\calN}
\newcommand{\hid}{\calH}

\newcommand{\advanced}{*}
%\newcommand{\advanced}{}



\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbS}{\mathbb{S}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

%\newcommand{\mya}{\mbox{a}}
%\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mathrm{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mathrm{train}}}
\newcommand{\dataTest}{\calD_{\mathrm{test}}}
\newcommand{\dataValid}{\calD_{\mathrm{valid}}}
\newcommand{\Xtrain}{\vX_{\mathrm{train}}}
\newcommand{\Xtest}{\vX_{\mathrm{test}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
%\newcommand{\data}{D}
\newcommand{\err}{\mathrm{err}}
\newcommand{\logit}{\mathrm{logit}}

% graph terms 
\newcommand{\nbd}{\mathrm{nbd}}
\newcommand{\nbr}{\mathrm{nbr}}
\newcommand{\anc}{\mathrm{anc}}
\newcommand{\desc}{\mathrm{desc}}
\newcommand{\pred}{\mathrm{pred}}
\newcommand{\mysucc}{\mathrm{suc}}
\newcommand{\nondesc}{\mathrm{nd}}
\newcommand{\pa}{\mathrm{pa}}
%\newcommand{\pa}{\pi}
\newcommand{\parent}{\mathrm{pa}}
\newcommand{\copa}{\mathrm{copa}}
\newcommand{\ch}{\mathrm{ch}}
\newcommand{\mb}{\mathrm{mb}}
\newcommand{\connects}{\sim}
\newcommand{\nd}{\mathrm{nd}}
\newcommand{\bd}{\mathrm{bd}}
\newcommand{\cl}{\mathrm{cl}}



\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}

%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}
%\newcommand{\inv}[1]{\ensuremath{\frac{1}{#1}}}
%\newcommand{\T}[1]{{\ensuremath{\left(#1\right)}}}
%\newcommand{\Tbr}[1]{{\ensuremath{\left[#1\right]}}}
%\newcommand{\Normal}[1]{\ensuremath{\mathpzc{N}\T{#1}}}
%\newcommand{\expof}[1]{\ensuremath{\exp\Tbr{#1}}}
%\newcommand{\So}{\ensuremath{\Rightarrow}}
%\newcommand{\ud}{\ensuremath{\mathrm{d}}}



\newcommand{\vfj}{\vf_j}
\newcommand{\vfk}{\vf_k}

\newcommand{\entropyBethe}{\mathbb{H}_{\mathrm{Bethe}}}
\newcommand{\entropyKikuchi}{\mathbb{H}_{\mathrm{Kikuchi}}}
\newcommand{\entropyEP}{\mathbb{H}_{\mathrm{ep}}}
\newcommand{\entropyConvex}{\mathbb{H}_{\mathrm{Convex}}}

\newcommand{\freeEnergyBethe}{F_{\mathrm{Bethe}}}
\newcommand{\freeEnergyKikuchi}{F_{\mathrm{Kikuchi}}}
\newcommand{\freeEnergyConvex}{F_{\mathrm{Convex}}}

\newcommand{\sigmaMle}{\hat{\sigma}^2_{mle}}
\newcommand{\sigmaUnb}{\hat{\sigma}^2_{unb}}


%**********************************
\newcommand{\keywordSpecial}[2]{{\bf #1}\index{keywords}{#2@#1}}
\newcommand{\bfidx}[1]{{\bf #1}}
%\newcommand{\keywordDef}[1]{{\bf #1}\index{keywords}{#1|bfidx}}
\newcommand{\keywordDefSpecial}[2]{{\bf #1}\index{keywords}{#2@#1|bfidx}}

\newcommand{\keywordDef}[1]{{\color{Blue}{\bf #1}}}


%\newcommand{\keywordDef}[1]{{\bf #1}}

==> embedding_arxiv/randomForests.tex <==
%\note{FH: I was somewhat confused when I read this section the first time; Nando, since you know the domain well could you maybe have a look?}

The work of Shotton et al. \cite{Shotton:2011} demonstrated state-of-the-art real-time human pose estimation from depth images by classifying each pixel with a body part class.  The ground truth body part labels and corresponding depth image are visualized in Figure \ref{fig:rf-all}~(left). Following Shotton et al \cite{Shotton:2011}, the random forest classifier is trained with synthetic data.  Pairs of depth and labeled images are generated using open datasets and graphics packages. For this experiment, we used random poses from the CMU mocap database to generate two hundred pairs of 320x240 resolution depth and body part images.  

The feature space is the difference of depth between pairs of pixels.  The location of each pixel in the pair is specified as an offset from the pixel being classified. The center diagram of Figure \ref{fig:rf-all} shows one feature for the pixel in the green box.  The pixel location in the red box is specified by offset u and the pixel in the white box is specified by offset v.  By scaling the offsets u,v by the depth of the pixel being classified, the features are depth invariant.  The two offsets and threshold make up the five parameters of each node in the tree.  
%\note{FH: I guess an offset has two coordinates? In that case, I'd replace ``specified by offset u'' by ``specified by the 2-dimensional offset u'' for clarity.}
The tree is built using the standard approach of recursively constructing each node by selecting the offsets and threshold that maximizes the information gain; see \cite{Shotton:2011}
for more details.

Candidate offsets are drawn from a 2d Gaussian.  If the variance is low then the random forest classifier is learning local features.  If the variance is the high, the classifier is learning global features.  The candidate Gaussians for u and v are parameterized independently along with 4 other hyper parameters resulting in a total of 14 hyper-parameters.  The ranges for each parameter can be found in Table \ref{table:rf}.

For these experiments, the random forest classifier was trained from 100\,000 random pixels from the 140 pose training set. Including the background class, there were 5\,000 samples per body part class.  The random forest accuracy across all 4.6 million pixels in a 60 pose test set is plotted in the right of Figure~\ref{fig:rf-all}. 
Random search performed remarkably well at this task, clearly outperforming pure BO. However, REMBO performed yet better than Random. More importantly, REMBO found a parameter configuration that performed better than previous manual tuning.    
%\note{FH: Dave, could one say that that manual tuning was really tedious (optimally quantify the human time spent) or was done by experts, or matters a lot in practice? That would make this argument stronger...}


\begin{table}[t]
\caption{Hyperparameter ranges for random forest classifier}
\label{table:rf}
\begin{center}
{\footnotesize
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf Parameter}  &\multicolumn{1}{c}{\bf Range}
\\ \hline \\
Number of candidate offsets at each node         &[5 1000] \\
Minimum samples for non-leaf nodes             &[1 50] \\
Maximum depth of the tree             &[2 20] \\
Number of trees in forest             &[1 10] \\
X, Y mean of candidate offsets             &[-200 200]\\
X, Y and XY variance  of candidate offsets           &[0.0 300]\\
\end{tabular}
}
\end{center}
\vspace{-1.5em}
\end{table}

%\note{FH: Dave, are all the samples treated as lying on a uniform scale, or are some log-transformed? E.g. `Number of candidate offsets to try at each node' or `Minimum samples for non-leaf nodes'?}


\begin{figure}[t]
\centering
  \raisebox{0.6cm}{\includegraphics[height=0.2\textheight]{figures/rf-all-nips-cropped.png}} \vspace{0.25em}
  \raisebox{0.6cm}{\includegraphics[height=0.2\textheight]{figures/rf-all-nips-offsets.png}} \vspace{0.25em}
     \includegraphics[scale=0.38]{figures/rf.png}
  \caption{Ground truth depth, ground truth body parts and predicted body parts (left), features specified by offsets u and v (middle) and the plot of prediction accuracy (right).  REMBO selected better hyperparameter settings than both Random and Random.}
  \label{fig:rf-all}
\end{figure}


==> embedding_arxiv/randomForests2.tex <==
We now evaluate REMBO's performance for optimizing the 14 parameters of a random forest body part classifier. This classifier closely follows the proprietary system used in the Microsoft Kinect \cite{Shotton:2011} and is available at \url{https://github.com/david-matheson/rftk}.

We begin by describing some details of the dataset and classifier in order to build intuition for the objective function and the parameters being optimized. The data we used consists of pairs of depth images and ground truth body part labels. Specifically, we used 1\,500 pairs of 320x240 resolution depth and body part images, each of which was synthesized from a random pose of the CMU mocap dataset. Depth, ground truth body parts and predicted body parts (as predicted by the classifier described below) are visualized for one pose in Figure \ref{fig:rf-all}~(left). There are 19 body parts plus one background class. 
For each of these 20 possible labels, the training data contained 25\,000 pixels, randomly selected from 500 training images. Both validation and test data contained \emph{all} pixels in the 500 validation and test images, respectively.

\begin{figure}[t]
\centering
  \raisebox{0.6cm}{\includegraphics[height=0.2\textheight]{figures/rf-all-nips-cropped.png}} 
  ~~~~~~~~~~
  \raisebox{0.6cm}{\includegraphics[height=0.2\textheight]{figures/rf-all-nips-offsets.png}} 
  \caption{Left: ground truth depth, ground truth body parts and predicted body parts; Right: features specified by offsets u and v.}
  \label{fig:rf-all}
\end{figure}

The random forest classifier is applied to one pixel $P$ at a time. At each node of each of its decision trees, it computes the depth difference between two pixels described by offsets from $P$ and compares this to a threshold. 
At training time, many possible pairs of offsets are generated at random, and the pair yielding highest information gain for the training data points is selected. Figure \ref{fig:rf-all}~(right) visualizes a potential feature for the pixel in the green box: it computes the depth difference between the pixels in the red box and the white box, specified by respective offsets u and v.
%By scaling the offsets u and v by the depth of the pixel being classified, the features are depth invariant. 
At training time, u and v are drawn from two independent 2-dimensional Gaussian distributions, each of which is parameterized by its two mean parameters $\mu_1$ and $\mu_2$ and three covariance terms $\Sigma_{11}$, $\Sigma_{12}$, and $\Sigma_{22}$ ($\Sigma_{21}=\Sigma_{12}$ because of symmetry). 
These constitute 10 of the parameters that need to be optimized, with range [-50,50] for the mean components and [1, 200] for the covariance terms. Low covariance terms yield local features, while high terms yield global features. 
%
Next to these ten parameters, the random forest classifier has four other standard parameters, outlined in Table \ref{table:rf}. 
%
It is well known in computer vision that many of the parameters described here are important. Much research has been devoted to identifying their best values, but results are dataset specific, without definitive general answers.

\begin{table}[t]
\caption{Parameter ranges for random forest classifier. For the purpose of optimization, the maximum tree depth and the number of potential offsets were transformed to log space.}
\label{table:rf}
\begin{center}
{\footnotesize
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf Parameter}  &\multicolumn{1}{c}{\bf Range}
\\ \hline \\
Max. tree depth         &[1 60] \\
Min. No. samples for non leaf nodes             & [1 100]  \\
No. potential offsets to evaluate           &[1 5000] \\
Bootstrap for per tree sampling           &[T F] \\
\end{tabular}
}
\end{center}
\end{table}



%Each tree was trained with 500\,000 samples. However, for computational efficiency, at each node only a random subset of samples is considered. 
%with thresholds at a rate of 0.001 and a cap of 100. 
%This node subsampling allowed for complex forests to be learnt within the 5 minute budget. 

The objective in optimizing these RF classifier parameters is to find a parameter setting that learns the 
best classifier in a given time budget of five minutes. To enable competitive performance in this short amount of time, at each node of the tree only a random subset of data points is considered.
Also note that the above parameters do not include the number of trees $T$ in the random forest; since performance improves monotonically in $T$, we created as many trees as possible in the time budget. Trees are constructed depth first and returned in their current state when the time budget is exceeded. 
Using a fixed budget results in a subtle optimization problem because of the complex interactions between the various parameters (maximum depth, number of potential offsets, number of trees and accuracy). 

It is unclear a priori whether a low-dimensional subspace of these 14 interacting parameters exists that captures the classification accuracy of the resulting random forests. 
We performed large-scale computational experiments with REMBO, random search, and standard Bayesian optimization (BO) to study this question. In this experiment, we used the high-dimensional kernel for REMBO to avoid the potential over-exploration problems of the low-dimensional kernel described in Section~\ref{sec:choice_of_kernel}. We believed that $D=14$ dimensions would be small enough to avoid inefficiencies in fitting the GP in $D$ dimensions. This belief was confirmed by the observation that standard BO (which operates in $D=14$ dimensions) performed well for this problem. 
%REMBO, by working on only a subspace of the domain of BO, should converge faster to the optimizer that falls within its domain.
%Each run of each method required over 80 hours on a dual core machine, making the total computation time for this experiment over 2400 hours on a dual core machine. 


\begin{figure}[t]
\centering
%   \includegraphics[scale=0.38]{figures/rf.png} % FH: there is a bug, this is just a copy of rf_interleave.png with different colours. It's fine now, only the naming of the files is awkward.
   \includegraphics[scale=0.41]{figures/rf_original.png}
%   \includegraphics[scale=0.38]{figures/rf_interleave.png}
   \includegraphics[scale=0.41]{figures/rf.png}
  \caption{Performance of various methods for optimizing RF parameters for body part classification. For all methods, we show RF accuracy (mean $\pm$ 1/4 standard deviation across 10 runs) for all 2.2 million non background pixels in the 500-pose validation set, using the RF parameters identified by the method. The results on the test set were within 1\% of the results on the validation set.  Left: performance with a single run of each method; Right: performance with $k=4$ interleaved runs.}
  \label{fig:rf-results}
\end{figure}


Figure \ref{fig:rf-results} (left) shows the results that can be obtained by a single run of random search, BO, and REMBO. Remarkably, REMBO clearly outperformed random search, even based on as few as $d=3$ dimensions.\footnote{Due to the large computational expense of this experiment (in total over half a year of CPU time), we only performed conclusive experiments with $d=3$; preliminary runs of REMBO with $d=4$ performed somewhat worse than those with $d=3$ for a budget of 200 function evaluations, but were still improving at that point.}
However, since the extrinsic dimensionality was ``only'' a moderate $D=14$, standard Bayesian optimization performed well, and since it was not limited to a low-dimensional subspace it outperformed REMBO. 
%
Nevertheless, several REMBO runs actually performed very well, comparably with the best runs of BO. Consequently, when running $k=4$ interleaved runs of each method, REMBO performed almost as well as BO, matching its performance up to about 450 function evaluations (see Figure \ref{fig:rf-results}, right). 

We conclude that the parameter space of this RF classifier does not appear to have a clear low effective dimensionality;
since the extrinsic dimensionality is only moderate, this leads REMBO to perform somewhat worse than standard Bayesian optimization, but it is still possible to achieve reasonable performance based on as little as $d=3$ dimensions. 



%From previous work, we knew that all 14 parameters were important but it was unknown if the parameter space was a rotated low dimensional embedding. The success of BO with respect to REMBO is evidence that this problem does not have a low effective dimension. 
%Consequently, a random embedding no longer has high probability of containing the optimum. This is supported by REMBO having high variance across runs and converging to a suboptimal solution in expectation. Even without low effective dimensionality a 3 dimensional embedding in a 14 dimensional space is able to achieve results that are within 2\% of BO in expectation. If other applications parameter spaces are of such high dimension that BO can not be applied, the results of this experiment gives hope to REMBO achieving reasonable results even if the problem domain does not have low effective dimensionality.

%FH: This paragraph was a little outdated. I added references to how you would actually do what we argue for. But the paragraph is tangential to the paper and we did not actually even release the source code for the RFs, let alone the function samples. So in the end I dropped the paragraph alltogether.
%This experiment also shows that automatic configuration techniques can reveal scientific facts about the problem; for example how to choose the depth of trees in RFs. For this reason, we feel it is important to advance to the machine learning community the following message about methodology. For any specific dataset, if researchers were to release the obtained objective function evaluations, other researchers could use these values to expedite their experiments and gain greater knowledge about the problem domain. For example, our experiments with RFs took many days with powerful clusters of computers. Other researchers could build on this data and ultimately learn a model for the objective function in this domain and, therefore, understand how the random forests parameters and design choices interact and affect performance \cite<for example, using the methods described by>{Hutter:2014}. Based on this data, we could also create surrogate optimization problems~\cite{Eggensperger2015} that resemble the original problem but are substantially cheaper to work with. To facilitate such meta-analyses, every expensive function evaluation should be made to count in an online database, such as OpenML~\cite{Vanschoren:2013:2641190.2641198}.




==> embedding_arxiv/regret.tex <==
%!TEX root = embedding.tex
% RegretBounds.tex

% When using the high-dimensional kernel $k^D$ on $\{p_{\mathcal{X}}(\vA\vy): \vy \in {\cal Y} \} \subset {\cal X}$, we could easily apply previous theoretical results \cite{Srinivas:2010,Bull:2011,deFreitas:2012}. However, this is not satisfying since the rates of convergence would still depend on $D$. If the low-dimensional embedding captures the optimizer, and since the search is conducted in $\{p_{\mathcal{X}}(\vA\vy): \vy \in {\cal Y} \}$ instead of ${\cal X}$, we should expect faster rates of convergence that only depend on the size of the embedding's dimensionality. The rest of this section shows that it is indeed possible to obtain rates of convergence that only depend on the embedding's dimensionality.
%These faster rates would then agree with what we observe in practice. 

In this section, we provide regret results for REMBO in the special case that (1)~the embedded subspace has the same dimension as the effective dimension and (2)~the embedded subspace contains a maximum of the function $f$ inside the box $\mathcal{X}$. More specifically, here we will analyze a simplified version of the algorithm that performs Bayesian optimization only inside the box $\mathcal{X}$ rather than considering its extension beyond $\mathcal{X}$ and projecting onto the boundary of $\mathcal{X}$ as done in our actual implementation. 

We acknowledge that this mismatch between the theoretical results and our actual algorithm is rather unsatisfactory. However, some of the obstacles that stand in the way of a complete analysis of the algorithm are currently insurmountable, since they would require the development of new tools that are far beyond the scope of this paper. We point these out at the end of this section and hope that our partial result will motivate the development of such tools, which might not otherwise receive any attention from the community.

We begin our mathematical treatment with the definitions of \emph{simple regret} and the \emph{skew squared exponential (SSE)} kernel.
\begin{mydefinition}\label{def:regret} Given a function $f: {\mathcal{X}} \to \mathbb{R}$ and a sequence of points $\{\vx_t\}_{t=1}^\infty \subseteq \mathcal{X}$, the \emph{simple regret} {\bf with respect to the set} $\mathcal{X}$ at time $T$ is defined to be $r_f(T) =  \sup_{\mathcal{X}}f - \displaystyle\max_{t=1}^T f(\vx_t)$.
\end{mydefinition}
\begin{mydefinition}\label{def:ssekernel}
Given a symmetric, positive-definite matrix $\mathbf{\vDelta}$ 
and $K_{SE}$, we define the corresponding \emph{skew squared exponential} kernel as
$$ k_{\vDelta}(\vy^{(1)},\vy^{(2)}) = 
K_{SE}\left(\mathbf{\vDelta}^{-1/2} (\vy^{(1)}-\vy^{(2)})\right). $$
\end{mydefinition}
Given $\vDelta$,
% \note{FH: in the current text $\ell$ does not factor in anywhere, so if we leave this as is we should also drop the part ``$\ell$ (as in the squared exponential kernel $k_{\ell}^d$) ''. But there is also commented text in the source referring to $k_\ell$; we might want to include something of that (and in that case leave in the part about $\ell$).}
and $\mathcal{X} \subseteq \mathbb R^d$, we denote the Reproducing Kernel Hilbert Spaces (RKHSs) corresponding to $k_{\vDelta}$ by $\calH_{k_{\vDelta}}$ \cite[Definition 4.18]{Steinwart:2008}.
Note that for the setting $\vDelta = \ell^2 I$ we recover the squared exponential kernel $k_{\ell}^d$ introduced earlier.
% and $k_\ell$ by $\calH_{k_{\vDelta}}(\mathcal{X})$ and $\calH_\ell(\mathcal{X})$, respectively \cite[Definition 4.18]{Steinwart:2008}. Moreover, given an arbitrary kernel $k_{\vDelta}$, we will denote its RKHS by $\calH_{k_{\vDelta}}$.
To simplify notation, we introduce yet another definition.
\begin{mydefinition}\label{def:canrep}
Consider the function $f: \calS \rightarrow \mathbb{R}$, where $\calS \subset \mathbb{R}^D$
is a $d$-dimensional subspace of $\mathbb{R}^D$. 
Let $\vPhi \in \mathbb{R}^{D \times d}$ be a matrix 
whose columns form an orthonormal basis for ${\cal S}$.
We define the \emph{canonical representation} $\overline{f}: \mathbb{R}^d \rightarrow \mathbb{R}$ 
of $f$ as $\overline{f}(\vx) = f(\vPhi \vx)$.
\end{mydefinition}

Our main result below shows that the simple regret of a variation of REMBO vanishes with rate $\mathcal O(t^{-\frac{1}{d}})$ with high probability. This REMBO variant uses a fixed kernel parameter length scale $\ell$ and, more importantly, restricts its search to its embedding inside the box $\mathcal{X}$.
 
We only make the assumption that the cost function restricted to $\mathcal T$ is governed by a skew squared exponential kernel, a much weaker assumption than the standard assumption that the cost function is governed by an axis aligned kernel in $D$ dimensions \cite<see, e.g.,>{Bull:2011}. Despite the fact that the cost function restricted to $\mathcal T$ is governed by a skew squared exponential kernel, the result shows that we can control the regret using the low-dimensional squared exponential kernel.

\begin{theorem}\label{thm:regret}
Let $\mathcal{X} \subset \mathbb{R}^D$ be a compact subset with non-empty interior that is convex and contains the origin and $f:\mathbb{R}^D \to \mathbb{R}$, a function with effective dimension $d$. 
Suppose that the canonical representation of the restriction of $f$ to its effective subspace $\mathcal T$, denoted $\overline{f|_\mathcal T}$, is an element of the RKHS $\calH_{k_{\vDelta}}(\mathbb R^d)$ with $\vDelta$ symmetric and positive definite and also satisfying $0 < r^2 < \lambda_{\min}(\vDelta) \leq \lambda_{\max}(\vDelta) < R^2$ for constants $r$ and $R$, where $\lambda_{\min}(\vDelta)$ and $\lambda_{\max}(\vDelta)$ are the extreme eigenvalues of $\vDelta$.

Let $\vA$ be a $D \times d$ matrix, whose elements are drawn from the normal distribution $\mathcal N\left(0,1\right)$. 
%Supposing that the image of $\vA$ intersects the maximum locus of $f$ inside the set $\mathcal{X}$, 
Then, given any $\epsilon > 0$, we can choose a length-scale $\ell = \ell(\epsilon)$ such that running REMBO with kernel $k^d_{\ell}$ on the restriction of $f$ to the image of $\vA$ inside $\mathcal{X}$ has simple regret {\bf with respect to the set} $\textup{Im } \vA \cap \mathcal{X}$ in $\mathcal O(t^{-\frac{1}{d}})$ with probability $1-\epsilon$.
\end{theorem}

This theorem does not follow directly from the results of \citeA{Bull:2011}, since the kernel is not aligned with the axes, both in the high-dimensional space and the lower dimensional embedding. 
%Thus, even given the true length scale the aforementioned paper will not entail a convergence result.

Please refer to Appendix \ref{sec:regret_proof} for the proof of this theorem. 
The general idea of the proof is as follows. If we have a squared exponential kernel $k_\ell$, with a smaller length scale than a given kernel $k_{\vDelta}$, then an element $f$ of the RKHS of $k_{\vDelta}$
% , considered as a function $f:\mathcal X \to \mathbb R$, 
is also an element of the RKHS of $k_\ell$ (see Lemma~\ref{lem:bull4} in the Appendix for more details). 
% \note{FH: this fact was repeated in the next subsection. I removed that occurrence, but let's put in a reference for it.}
% with the difference in the two norms being bounded. 
So, when running expected improvement, one can safely use $k_\ell$ instead of $k_{\vDelta}$ as the kernel and still obtain a regret bound. Most of the proof is dedicated to finding a length scale $\ell$ that fits ``underneath'' our kernel, so we can replace our kernel with $k_\ell$, to which we can apply the results of \citeA{Bull:2011}.

Note that in the above theorem we make the assumption that the embedded dimension and the effective dimension are equal to each other. Given bounds such as Proposition 1 of \citeA{deFreitas:2012}, we strongly believe that a similar result holds when the embedded dimension is higher than the effective dimension; however, the analysis of that setting remains elusive due to the fact that none of the methods available in the literature on regret bounds for Bayesian optimization algorithms can handle kernels that have flat dimensions (i.e. when $\vDelta$ is not positive-definite), and adapting them to such a case requires tools from statistics that have yet to be developed. Given that, theoretical bounds for the case with $d_e < d$ are outside the scope of this work.

%\masrour{
Moreover, note that this theorem provides a sublinear regret result for REMBO with respect to the whole set $\mathcal{X}$ only in the situation that $\textup{Im }\vA$ intersects the maximum locus of the function $f$ \emph{inside} the set $\mathcal{X}$. Note that Theorem \ref{prop:2} provides a lower bound on the probability of this happening in the special case that the effective subspace is axis-aligned.
%} %
%
Proving regret bounds for situations in which the image of $\vA$ only contains a maximum outside of $\mathcal{X}$ would require dealing with the RKHS of non-stationary kernels, since the projection operator $p_{\mathcal{X}}$ can have non-constant Jacobian. This is related to the situation with treed GPs~\cite{Gramacy:2004}, with the additional, immensely complicating ingredient that is the continuity assumption imposed along the boundaries of the various partitions of the space (since $p_{\mathcal{X}}$ is continuous). Similar to the theory of Partial Differential Equations, where boundary conditions are the hardest part of the problem, we anticipate this modification to be a non-trivial, albeit very interesting, undertaking, and pose it as an open problem to the community.

% The above theorem requires the embedded dimension and the effective dimension to coincide, but due to Proposition 1 of \citeA{deFreitas:2012}, we strongly believe that the analysis of \citeA{Bull:2011} can be modified to allow for situations in which some of the automatic relevance determination (ARD) parameters are zero, which is precisely what is preventing us from extending this result to the case where $d > d_e$.
% when the embedded dimension $d$ is higher than the effective dimension $d_e$. We defer this non-trivial extension to future work.

\begin{remark}
The above theorem would also hold for a class of stationary kernels which includes 
the popular Mat\'ern kernel. 
For conciseness of presentation, we do not include this result, but refer 
the curious reader to~\citeA{Bull:2011} for more details.
\end{remark}



==> embedding_arxiv/regretproof.tex <==
%!TEX root = embedding.tex
Before embarking on the proof of Theorem \ref{thm:regret}, 
we introduce some definitions and state a few preliminary results,
which we quote from \citeA{Bull:2011} to facilitate the reading of this exposition.

% \begin{lemma}[Lemma 4.6 in \cite{Steinwart:2008}]\label{lem:Steinwart4.6} Let $k_1$ be a kernel on $\mathcal{X}_1$ and $k_2$ be a kernel on $\mathcal{X}_2$. Then $k_1 \cdot k_2$ is a kernel on $\mathcal{X}_1 \times \mathcal{X}_2$.
% \end{lemma}
% 
% \begin{remark}\label{rmk:Steinwart4.6} In the proof of the above lemma in \cite{Steinwart:2008}, it is argued that if $\calH_i$ is the RKHS of $k_i$ for $i=1,2$, then $\calH_1 \widehat\otimes \calH_2$ is the RKHS of $k_1 \cdot k_2$, where $\widehat\otimes$ is the tensor product of Hilbert spaces and the elements of $\calH_1 \widehat\otimes \calH_2$ have the form $h(x_1,x_2) = \sum_i f_i(x_1) g_i(x_2)$, where the functions $f_i: \mathcal{X}_1 \to \mathbb{R}$ are elements of $\calH_1$ and the functions $g_i: \mathcal{X}_2 \to \mathbb{R}$ are elements of $\calH_2$.
% \end{remark}
% 
% \begin{corollary}[Corollary 4.43 in \cite{Steinwart:2008}]\label{cor:Steinwart4.43} Given $\mathcal{X} \subseteq \mathbb R^d$ with non-empty interior, and $r > 0$, then we have an isomorphism of Hilbert spaces $\mathcal H_r(\mathcal{X}) \cong \mathcal H_r(\mathbb R^d)$, through an extension operator $I_\mathcal{X}$ (whose definition is omitted, since it is not needed here).
% \end{corollary}
% 
% \begin{proposition}[The second part of Proposition 4.46 in \cite{Steinwart:2008}]\label{prop:Steinwart4.46} Given $0 < \ell < U$, for all non-empty $\mathcal{X} \subseteq \mathbb{R}^d$, the RKHS $\calH_{U}(\mathcal{X})$ can be mapped under the identity map into $\calH_{\ell}(\mathcal{X})$ and we have the following bound:
% \[ \left\| \textup{id} : \calH_{U} \to \calH_{\ell} \right\| \leq \left( \frac{U}{\ell} \right)^{\frac{d}{2}}, \]
% where the norm in the equation is the operator norm, i.e. $\sup_{f \in \calH_{U}} \frac{\|f\|_{\mathcal H_\ell}}{\|f\|_{\mathcal H_U}}$.
% \end{proposition}
% 
% \begin{remark} Note that here, the map $\textup{id}$ signifies the following: the element $f \in \calH_U$ corresponds to a real-valued function on $\mathcal{X}$, which we will also denote by $f$, so one can pose the question whether or not this function is an element of $\calH_\ell$ as well, and the existence of the map $\textup{id}: \calH_{U} \to \calH_{\ell}$ implies that $f$ is indeed an element of $\calH_{\ell}$. 
% Equivalently, $\calH_{U} \subset \calH_{\ell}$ and
% \[
% \|f\|_{\calH_{\ell}} \leq \left( \frac{U}{\ell} \right)^{\frac{d}{2}} \|f\|_{\calH_{U}}.
% \]
% In the proof of our theorem below, we will extend this result for squared exponential kernels to skewed squared exponential kernels.
% \end{remark}
We denote the Fourier transform of any function 
$\phi(\vx)$ as $\widehat{\phi}(\vxi) = \int_{\mathbb{R}^d}{e^{-2\pi i \vx^T \vxi}\phi(\vx)d\vx}$.
In this section we consider kernels of the form
$$
k_{\vDelta}(\vx^{(1)}, \vx^{(2)}) =  
K_{\vDelta}(\vx^{(1)}-\vx^{(2)}) = 
K(\vDelta^{-\frac{1}{2}} (\vx^{(1)}-\vx^{(2)}))
$$
where $\vDelta$ is a positive definite matrix and $K$ has Fourier transform 
$\widehat{K}$
% $ = \int_{\mathbb{R}^d}{e^{-2\pi i \vx^T \vxi}K(\vx)d\vx}$
% \note{FH: I replaced $\vxi$ by $\vxi$ and $<\vxi,\vx>$ by $\vx^T \vxi$ -- although the former is one standard notation it would be the only place in the paper where we use it and we'd have to introduce it. I have not replaced $\vxi$ by $\vxi$ in the remainder since I wanted to give you a chance to undo it if you disagree.}
such that $\widehat{K}$ is isotropic and radially non-increasing.
Notice that both the squared exponential kernel and the skew squared exponential
kernel introduced in Definition \ref{def:ssekernel} of the main text are represented in the form above.
The popular kernels from the Mat\'ern class can also be represented in this form. 
In general, the results in this section would follow for any kernel
that satisfies the four assumptions detailed by~\citeA{Bull:2011}.
\begin{lemma}[Lemma 1 of \citeA{Bull:2011}]
 \label{lem:bull1}
 $\calH(\mathbb{R}^d)$ is the space of real continuous functions 
 $f \in L^2(\mathbb{R}^d)$ whose norm
 $$
 \|f\|^2_{\calH(\mathbb{R}^d)} := 
 \int{\frac{ | \widehat{f}(\vxi) |^2 }{\widehat{K}(\vxi)}d\vxi}
 $$
 is finite, taking $0/0=0$.
 % Here $\widehat{f}$ is the Fourier transform of $f$.
\end{lemma}
% \note{FH: what is $\widehat{f}$ in that lesmma?}

\begin{lemma}[Lemma 2 of \citeA{Bull:2011}]
 \label{lem:bull2}
 Given a set $\calS \subseteq \mathbb{R}^d$,
 $\calH(\calS)$ is the space of functions $f = g|\calS$ ($f$ is $g$ restricted to $\calS$) 
 for some $g \in \calH(\mathbb{R}^d)$, with norm
 $$
 \|f\|_{\calH(\calS)} := \inf_{g|\calS = f} \|g\|_{\calH(\mathbb{R}^d)},
 $$
 and there is a unique $g$ minimizing this expression.
\end{lemma}
% \note{FH: I'm confused by ``$f = g|s$ ($f$ is $g$ restricted to $\calS$)''. Does $s$ just stand for $\calS$, or is it something new? If the former, can we just write $g|\calS$?}

\begin{lemma}[Lemma 4 of \citeA{Bull:2011}, extended to our setting]
 \label{lem:bull4}
 Let $\calS \subseteq \mathbb{R}^d$
 and $\vDelta$ and $\vDelta'$ be two symmetric positive definite matrices.
 Let $\lambda_{\max}( \vDelta') $, $ \lambda_{\min}(\vDelta)$ 
 be the largest and the smallest eigenvalues of $\vDelta'$, $\vDelta$ respectively
 such that $\lambda_{\max}( \vDelta') \leq \lambda_{\min}(\vDelta)$.
 Then $f \in \calH_{k_{\vDelta}}(\calS)$  implies 
 $f \in \calH_{k_{\vDelta'}}(\calS)$ 
 and also
 $$\|f\|_{\calH_{k_{\vDelta'}}(\calS)} 
 \leq \left(\frac{| \vDelta | }{ | \vDelta'|}\right)^{\frac{1}{2}} 
 \|f\|_{\calH_{k_{\vDelta}}(\calS)}$$
 where $|\vDelta|$ is the determinant of $\vDelta$.
% \note{FH: As stated, this lemma is confusing since it allows two interpretations:
% ``A given B and C'' can mean ``(A if B) and C'', or A if (B and C).''.
% I'd reword to 
%  If $\lambda_{\max}( \vDelta') \leq \lambda_{\min}(\vDelta)$ then
%  $f \in \calH_{k_{\vDelta}}(\calS)$ implies $f \in \calH_{k_{\vDelta'}}(\calS)$ and ...}
\end{lemma}
\begin{proof}
 Since $\vDelta$ and $\vDelta'$ are positive definite we can write 
 $\vDelta = Q^T \Sigma Q$ and $\vDelta' = Q'^T \Sigma' Q'$ 
 where $Q$ and $Q'$ are orthonormal.
 Let $C = \left(\frac{| \vDelta' | }{ | \vDelta|}\right)^{\frac{1}{2}}$. 
 Since $\lambda_{\max}( \vDelta') \leq \lambda_{\min}(\vDelta)$, we know that 
 $$
 \|\Sigma'^{\frac{1}{2}} Q' \vxi \|^2
 =    \vxi^T \vDelta' \vxi 
 \leq \vxi^T \vDelta \vxi
 =    \|\Sigma^{\frac{1}{2}} Q \vxi \|^2.
 $$
 As $\widehat{K}$ is isotropic and radially non-increasing,
 we have that 
% \note{FH: sorry, what do the first and last equalities following from?}
 $$
 \widehat{K_{\vDelta'}}(\vxi)
 =    |\vDelta'|^{\frac{1}{2}} \widehat{K}( \Sigma'^{\frac{1}{2}}Q'\vxi) 
 \geq |\vDelta'|^{\frac{1}{2}} \widehat{K}( \Sigma^{\frac{1}{2}}Q\vxi)
 =    |\vDelta'|^{\frac{1}{2}} |\vDelta|^{-\frac{1}{2}} \widehat{K_{\vDelta}}(\vxi)
 =    C \widehat{K_{\vDelta}}(\vxi)
 $$
 where the first and the second last equality follows from the following property of Fourier transforms: $\widehat{h}(\vxi) = \frac{1}{|M|}\widehat{f}(M^{-T}\vxi)$ 
 if $h(\vx) = f(M\vx)$ given a non-singular matrix $M$.
 % $\widehat{f(Ax)} = \frac{1}{|A|^{1/2}}\widehat{f(x)}$.
 Given $f \in \calH_{k_{\vDelta}}(\calS)$, let $g \in \calH_{k_{\vDelta}}(\mathbb{R}^d)$
 be its minimum norm extension, as in Lemma~\ref{lem:bull2}. 
 By the definition of RKHS norm in Lemma~\ref{lem:bull1}, 
 $$
 \|f\|^2_{\calH_{k_{\vDelta'}}(\calS)} 
 = \|g\|^2_{\calH_{k_{\vDelta'}}(\mathbb{R}^d)}
 =    \int{\frac{ | \widehat{g} |^2 }{\widehat{K_{\vDelta'}}}}
 \leq \int{\frac{ | \widehat{g} |^2 }{C \widehat{K_{\vDelta}}}}
 =    C^{-1}\|f\|^2_{\calH_{k_{\vDelta}}(\calS)}.
 $$
 Since $C$ is finite, by Lemma~\ref{lem:bull1} we have that
 $f \in \calH_{k_{\vDelta}}(\calS)$  implies $f \in \calH_{k_{\vDelta'}}(\calS)$.
\end{proof}

\begin{figure}[t!]
\centering
  \includegraphics[width=0.8\textwidth]{figures/projection_kernels.pdf}
  \caption{A illustration of the different kernels defined in this proof. 
  In this figure, 
  the red line represents the one-dimensional space $\calY$ over which we optimize.
  The blue region is the original high-dimensional space. 
  The green line represents the effective subspace $\calT$ projected to a 
  one-dimensional space through $\vPi$. The true kernel $K_{\vDelta}$ is defined on 
  the green region. The true kernel on the high-dimensional space is then naturally
  $k^D = \vPi^*k_{\vDelta}$ and the true kernel on $\calY$ is
  $K_{\vDelta_d} = \vA^*k^D$. To optimize without the knowledge of $K_{\vDelta_d}$,
  we use a kernel $k_{\ell}$ which with high probability is thinner than 
  $K_{\vDelta_d}$ in all directions thus preserving convergence properties.}
  \label{fig:kernels}
\end{figure}

\begin{mydefinition}\label{pullback} Given a map $\pi: \mathcal{S} \to \mathcal{T}$ between any two sets $\mathcal{S}$ and $\mathcal{T}$, and any map $f: \underbrace{\mathcal{T} \times \cdots \times \mathcal{T}}_\text{$n$-times} \to \mathbb R$, with $n \geq 1$, we define the \emph{pull-back} of $f$ under $\pi$ as follows:
\[ \pi^* f(s_1, \ldots, s_n) := f\left(\pi (s_1), \ldots, \pi (s_n) \right). \]
% \note{FH: I'd rewrite $f(\pi s_1, \ldots, \pi s_n)$ as $f(\pi(s_1), \ldots, \pi(s_n))$, but didn't so to not mess with your notation if you don't like it.}
That is, one evaluates the pull-back $\pi^* f$ on points in $\mathcal{S}$ by first ``pushing them forward'' onto $\mathcal{T}$ and then using $f$ to get a number.

If the map $\pi$ is given by a matrix $\vA$, we will use the notation $\vA^* f$ for the pull-back of $f$ under the linear map induced by $\vA$. Moreover, given a matrix $\vA$ and a set $\mathcal{S}$ in its target space, we will denote by $\vA^{-1}(\mathcal{S})$ the set of all points that are mapped into $\mathcal{S}$ by $\vA$.
\end{mydefinition}

\begin{proposition}[Theorem 2 by \citeA{Bull:2011}, paraphrased for our particular setting]\label{thm:Bull} Given a squared exponential kernel $k_\ell$ on a compact subset $\mathcal Y \subset \mathbb R^d$ and a function $f \in \mathcal H_\ell(\mathcal Y)$, then applying Expected Improvement to $f$ results in simple regret that diminishes according to $\mathcal O\big(t^{-\frac{1}{d}}\big)$, with the constants worsening as the norm $\|f\|_{\mathcal H_\ell(\mathcal Y)}$ increases.
\end{proposition}

\begin{proof}[Proof of Theorem \ref{thm:regret}]
The proof of this result is structured into two parts.
In the first part of the proof, we give an analytic expression for the 
true kernel $k_{\vDelta_d}$ in the low dimensional space over which we optimize. 
In the second part of the proof, we show that this kernel is well-behaved with high probability
(specifically the maximum and minimum eigenvalues of $\vDelta_d$ are bounded above and below by constants depending on the probability of failure)
and apply Proposition~\ref{thm:Bull} to acquire the convergence rate.

Let $\vPhi \in \mathbb{R}^{D \times d}$ be a matrix, 
whose columns form an orthonormal basis for ${\cal T}$.
Let $\mathbf{\Pi}=\vPhi^T \vPhi \vPhi^T: \mathcal{X} \rightarrow \mathbb{R}^d$.
Note that $\mathbf{\Pi}$ is composed of an orthogonal projection from $\calX$ to $\calT$ and a bijective map from $\calT$ to $\mathbb{R}^d$. We will also denote the corresponding matrix by $\mathbf{\Pi}$. 

Recall from the theorem statement that $\overline{f|_{\mathcal T}}$ is assumed to be an element of the RKHS $\calH_{k_{\vDelta}}$, and that we have $f = {\vPi}^* \overline{f|_{\mathcal T}}$, i.e. $f$ is obtained from ``stretching $f|_{\mathcal T}$ open'' along the orthogonal subspace of $\mathcal T$. We can also define the kernel over $\mathbb{R}^D$ by $k^D := \mathbf{\Pi}^* k_{\vDelta}$.
%, defined by the formula
%\[ k_{\vDelta}(\vx^{(1)},\vx^{(2)}) = e^{(\vx^{(1)}-\vx^{(2)})^\top \mathbf{\vDelta}^{-1} (\vx^{(1)}-\vx^{(2)})}, \]
%for $\vx^{(1)},\vx^{(2)} \in \mathcal T$.

Now, given the embedding $\mathbb R^d \hookrightarrow \mathbb R^D$ defined by the matrix $\vA$, the pull-back function $\vA^* f$ is an element of the RKHS $\calH_{\vA^* k^D}$: Henceforth, we will use the notation 
\[ k_{\vDelta_d} := \vA^* k^D = \vA^* \mathbf{\Pi}^* k_{\vDelta} =  (\mathbf{\Pi}\vA)^* k_{\vDelta}. \]
In more detail, for $\vy^{(1)}, \vy^{(2)} \in \mathbb{R}^d$
\[ k_{\vDelta_d}(\vy^{(1)},\vy^{(2)}) = K\left((\vy^{(1)}-\vy^{(2)})^\top \vA^\top\mathbf{\Pi}^\top\mathbf{\vDelta}^{-1}\mathbf{\Pi}\vA (\vy^{(1)}-\vy^{(2)})\right).\]
For a pictorial illustration of the different kernels defined in this proof, 
please refer to Figure~\ref{fig:kernels}.

Since $\mathbf{\Pi}$ is an orthogonal projection matrix, it has an SVD decomposition $\mathbf{\Pi} = \vU\vS\vV$ consisting of an orthogonal $d\times d$ matrix $\vU$, an orthogonal $D \times D$ matrix $\vV$ and a $d \times D$ matrix $\vS$ that has the following form:
\[ \vS = \begin{bmatrix} 1 & 0 & \cdots & 0      & 0      & \cdots & 0 \\
                       0 & 1 & \cdots & 0      & 0      & \cdots & 0 \\
            \vdots & \vdots  & \ddots & \vdots & \vdots & \ddots & \vdots \\
                       0 & 0 & \cdots & 1      & 0      & \cdots & 0 \end{bmatrix}. \]
Now, given a fixed orthogonal matrix $\vO \in \mathbb{R}^{D \times D}$ and a random Gaussian vector $\vv \sim \mathcal N(\mathbf 0,\vI_{D \times D})$, due to the rotational symmetry of the normal distribution, the vector $\vO\vv$ is also a sample from $\mathcal N(\mathbf 0,\vI_{D \times D})$. Therefore, given a random Gaussian matrix $\Gamma$, $\vO\Gamma$ is also a random Gaussian matrix with the same distribution of entries. Moreover, given $\vS$ as above, $\vS\Gamma$ is a $d \times D$ random Gaussian matrix, since multiplying any matrix by $\vS$ on the left simply extracts the first $d$ rows of the matrix.

Given this, if we fix an orthogonal decomposition $\mathbf{\vDelta}^{-1} = \vP^\top \vD^{-1} \vP$, where $\vP$ is orthogonal and $\vD$ is a diagonal matrix with the eigenvalues of $\mathbf{\vDelta}$ along the diagonal, we can conclude that
\[ \vG := \vP\mathbf{\Pi}\vA = \vP\vU\vS\vV\vA  \]
%\note{NdF: It should be $\vG := \vP \mathbf{\Pi}\vA$ I think. MZ: Yes, you're right.}
is a random Gaussian matrix, and so the matrix 
$\mathbf{\vDelta}_d = \vA^\top\mathbf{\Pi}^\top\mathbf{\vDelta}^{-1}\mathbf{\Pi}\vA$
% \note{FH: did I overlook this, or is $\mathbf{\vDelta}_d$ undefined?}
can be decomposed into random Gaussian and diagonal matrices as follows:
\[ \mathbf{\vDelta}^{-1}_d = \vG^\top \vD^{-1} \vG. \]
Since random Gaussian matrices, as argued in the proof of Theorem~\ref{prop:1}, have full rank almost surely, $\mathbf{\vDelta}^{-1}_d$ is of full rank and is positive definite.


In the remainder of this proof, we replace $k_{\vDelta_d}$ with a kernel $k_\ell$ that is ``thinner'' than $k_{\vDelta_d}$ and so $\vA^* f$ is also an element of the RKHS of $k_\ell$. 
By showing that this is true, REMBO (which uses $k_\ell$) has enough approximation power. Moreover, the statement of Proposition~\ref{thm:Bull} applies.   

% Since $k^D$ is constant along $\mathcal T^\bot$, we get that $k_{\vDelta_d}$ is in turn constant along $\vA^{-1}\left(\mathcal T^\bot\right)$, and since $\vA$ is randomly chosen, the linear subspace $\vA^{-1}\left(\mathcal T^\bot\right)$ will almost surely be zero dimensional. Let us introduce the notation $\mathbf{\Pi}$ for the $d \times D$ matrix that projects vectors in $\mathbb R^D$ onto the effective subspace $\mathcal T$.

% We almost surely have that the $d \times d$ matrix $\mathbf{\Pi}\vA$ is non-singular, since the space of singular matrices has measure $0$, given the fact that it is the zero-set of a polynomial, namely the determinant. Therefore, the kernel $k_{\vDelta_d}$, which has the form
% \[ k_{\vDelta_d}(\vy^{(1)},\vy^{(2)}) = e^{(\vy^{(1)}-\vy^{(2)})^\top \vA^\top\mathbf{\Pi}^\top\mathbf{\vDelta}^{-1}\mathbf{\Pi}\vA (\vy^{(1)}-\vy^{(2)})} \]
% is also SSE, since $\vA^\top\mathbf{\Pi}^\top\mathbf{\vDelta}^{-1}\mathbf{\Pi}\vA$ is symmetric and positive definite, simply because of the symmetry and positive definiteness of $\mathbf{\vDelta}^{-1}$: given $\vy \neq 0$, we have 
% \[ \vy^\top \vA^\top\mathbf{\Pi}^\top\mathbf{\vDelta}^{-1}\mathbf{\Pi}\vA \vy = \widetilde\vy^\top \mathbf{\vDelta}^{-1} \widetilde\vy > 0, \]
% where  $\widetilde\vy := \mathbf{\Pi}\vA \vy \neq 0$ since $\mathbf{\Pi}\vA$ is invertible.
% In what follows, we will use the notation $\mathbf{\vDelta}_d := \left(\vA^\top\mathbf{\Pi}^\top\mathbf{\vDelta}^{-1}\mathbf{\Pi}\vA\right)^{-1}$. 

% Since $\mathbf{\Pi}$ is an orthogonal projection matrix, it has an SVD decomposition $\mathbf{\Pi} = \vU\vS\vV$ consisting of an orthogonal $d\times d$ matrix $\vU$, an orthogonal $D \times D$ matrix $\vV$ and a $d \times D$ matrix $\vS$ that has the following form:
% \[ \vS = \begin{bmatrix} 1 & 0 & \cdots & 0      & 0      & \cdots & 0 \\
%                        0 & 1 & \cdots & 0      & 0      & \cdots & 0 \\
%             \vdots & \vdots  & \ddots & \vdots & \vdots & \ddots & \vdots \\
%                        0 & 0 & \cdots & 1      & 0      & \cdots & 0 \end{bmatrix}. \]
% Now, given a fixed orthogonal matrix $\vO$ and a random Gaussian vector $\vv \sim \mathcal N(\mathbf 0,\vI_{D \times D})$, due to the rotational symmetry of the normal distribution, the vector $\vO\vv$ is also a sample from $\mathcal N(\mathbf 0,\vI_{D \times D})$. Therefore, given $\vO$ as above, and a random Gaussian matrix $\Gamma$, then $\vO\Gamma$ is also a random Gaussian matrix with the same distribution of entries. Moreover, given $\vS$ as above, $\vS\Gamma$ is a $d \times D$ random Gaussian matrix, since multiplying any matrix by $\vS$ on the left simply extracts the first $d$ rows of the matrix.

% Given this, if we fix an orthogonal decomposition $\mathbf{\vDelta}^{-1} = \vP^\top \vD^{-1} \vP$, where $\vP$ is orthogonal and $\vD$ is a diagonal matrix with the eigenvalues of $\mathbf{\vDelta}$ along the diagonal, we can conclude that
% \[ \vG := \vP\mathbf{\Pi}\vA = \vP\vU\vS\vV\vA  \]
% %\note{NdF: It should be $\vG := \vP \mathbf{\Pi}\vA$ I think. MZ: Yes, you're right.}
% is a random Gaussian matrix, and so the matrix $\mathbf{\vDelta}_d$ can be decomposed into random Gaussian and diagonal matrices as follows:
% \[ \mathbf{\vDelta}^{-1}_d = \vG^\top \vD^{-1} \vG. \]
Let $s_{\min}(\vM)$ and $s_{\max}(\vM)$ denote the smallest and the largest singular values of a matrix $\vM$. With this notation in hand, 
we point out the following two facts about concentration of singular values:
%\note{NdF: Does $s_{\max}(\vA)$ denote the largest singular value? MZ: Yes, I've added a note now.}
\begin{itemize}
\item[I.] Since for any pair of matrices $\vA$ and $\vB$, we have $s_{\max}(\vA\vB) \leq s_{\max}(\vA) s_{\max}(\vB)$, we get
\[ \frac{1}{\lambda_{\min}(\mathbf{\vDelta}_d)} = \lambda_{\max}(\mathbf{\vDelta}_d^{-1}) \leq s_{\max}(\vG)^2 s_{\max}(\vD^{-1}) \leq \frac{s_{\max}(\vG)^2}{r^2} \]
and since $\vG$ is a random matrix with Gaussian entries, we have (cf. Equation 2.3 by \citeA{Rudelson:2010})
\[ P\left(s_{\max} (\vG) < 2\sqrt{d}+t\right) \leq 1-2e^{-t^2/2}, \]
and so with probability $1-\frac{\epsilon}{2}$, we have
\[ s_{\max}(\vG) < 2\sqrt{d}+\sqrt{2\ln\frac{4}{\epsilon}}. \]

Therefore, with probability $1-\frac{\epsilon}{2}$, we have
\begin{equation}\label{eqn:LB}
 \lambda_{\min}(\mathbf{\vDelta}_d) > \left(\frac{r}{2\sqrt{d}+\sqrt{2\ln\frac{4}{\epsilon}}}\right)^2.
\end{equation}

Henceforth, we will use the notation
\[ \ell = \ell(\epsilon) := \frac{r}{2\sqrt{d}+\sqrt{2\ln\frac{4}{\epsilon}}} \]

\item[II.] On the other hand, we have
\[ \frac{1}{\lambda_{\max}(\mathbf{\vDelta}_d)} = \lambda_{\min}(\mathbf{\vDelta}_d^{-1}) \geq s_{\min}(\vG)^2 s_{\min}(\vD^{-1}) \geq \frac{s_{\min}(\vG)^2}{R^2} \]
together with the following probabilistic bound on $s_{\min}(\vG)$ (cf. Equation 3.2 by \citeA{Rudelson:2010}):
\[ P\left( s_{\min}(\vG) > \frac{\delta}{\sqrt{d}} \right) > 1 - \delta. \]
So, with probability $1-\frac{\epsilon}{2}$, we have
\[ s_{\min}(\vG) > \frac{\epsilon}{2\sqrt{d}}, \]
and so
\begin{equation}\label{eqn:UB}
 \lambda_{\max}(\mathbf{\vDelta}_d) < \frac{4dR^2}{\epsilon^2}
\end{equation}
holds with probability $1-\frac{\epsilon}{2}$.
%\note{NdF: Why 6 and not 4? MZ: Sorry, that was a typo.}

In what follows, we will use the notation:
\[ U = U(\epsilon) := \frac{2R\sqrt{d}}{\epsilon} \]
\end{itemize}

% Now, with these estimates in hand, we can go ahead and show that the following bound holds with probability $1-\epsilon$:



Now, with these estimates in hand, we have that by Lemma~\ref{lem:bull2}
and Lemma~\ref{lem:bull4}
the following bound holds with probability $1-\epsilon$:
\begin{equation}\label{eqn:RKHSNormBound}
\| \vA^*f \|_{\mathcal H_{\ell}(\vA^{-1}(\mathcal{X}))} 
\leq \| \vA^*f \|_{\mathcal H_{\ell}(\mathbb{R}^d)}
\leq \left(\frac{U(\epsilon)}{\ell(\epsilon)}\right)^{\frac{d}{2}} 
     \|\vA^* f\|_{\mathcal H_{\mathbf{\vDelta}_d}(\mathbb{R}^d)}
\end{equation}

Since the transformation $\mathbf{\Pi}\vA$ is invertible, we have that the map $(\mathbf{\Pi}\vA)^*: \mathcal H_{\mathbf{\vDelta}}(\mathbb R^d) \to \mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d)$ (recall that $k_{\mathbf{\vDelta}_d} = k_{(\mathbf{\Pi}\vA)^*\mathbf{\vDelta}}$) that sends $g \in H_{\mathbf{\vDelta}}$ to $(\mathbf{\Pi}\vA)^* g$ is an isomorphism of Hilbert spaces and so 
\begin{equation}\label{eqn:KernelIso}
\left\|\overline{f|_{\mathcal T}}\right\|_{\mathcal H_\mathbf{\vDelta}(\mathbb R^d)} = \|\vA^* f\|_{\mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d)}
\end{equation}
since we have $\vA^* f = \vA^* \left(\mathbf{\Pi}^* \overline{f|_{\cal T}}\right) = (\mathbf{\Pi}\vA)^* \overline{f|_{\cal T}}$.

By combining~\ref{eqn:RKHSNormBound} and~\ref{eqn:KernelIso}, we have that
$$
\| \vA^*f \|_{\mathcal H_{\ell}(\vA^{-1}(\mathcal{X}))} 
\leq \left(\frac{U(\epsilon)}{\ell(\epsilon)}\right)^{\frac{d}{2}} 
     \left\| \overline{f|_{\mathcal T}} \right\|_{\mathcal H_{\mathbf{\vDelta}}(\mathbb{R}^d)}.
$$

% This claim follows from the following sequence of facts:
% \begin{itemize}
% \item[A.] Since the transformation $\mathbf{\Pi}\vA$ is invertible, we have that the map $(\mathbf{\Pi}\vA)^*: \mathcal H_{\mathbf{\vDelta}}(\mathbb R^d) \to \mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d)$ (recall that $k_{\mathbf{\vDelta}_d} = k_{(\mathbf{\Pi}\vA)^*\mathbf{\vDelta}}$) that sends $g \in H_{\mathbf{\vDelta}}$ to $(\mathbf{\Pi}\vA)^* g$ is an isomorphism of Hilbert spaces and so 
% \begin{equation}\label{eqn:KernelIso}
% \|f|_{\mathcal T}\|_{\mathcal H_\mathbf{\vDelta}(\mathbb R^d)} = \|\vA^* f\|_{\mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d)}
% \end{equation}
% since we have $\vA^* f = \vA^* \left(\mathbf{\Pi}^* f|_{\mathcal T}\right) = (\mathbf{\Pi}\vA)^* f|_{\mathcal T}$.
% \item[B.] If we denote the eigenvalues of $\mathbf{\vDelta}_d$ by $\lambda_1 < \cdots < \lambda_d$, then, first of all, by Corollary \ref{cor:Steinwart4.43}, we have
% \[ \mathcal H_{\mathbf{\vDelta}_d}\left(\vA^{-1}(\mathcal{X})\right) \cong \mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d) \]
% and also by Remark \ref{rmk:Steinwart4.6}, we have the isomorphisms
% \begin{align*}
% \mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d) & \cong \mathcal H_{\sqrt{\lambda_1}}(\mathbb R) \;\hat\otimes \;\cdots\; \hat\otimes \;\mathcal H_{\sqrt{\lambda_d}}(\mathbb R) \\
% \mathcal H_{\ell}(\mathbb R^d) & \cong \mathcal H_{\ell}(\mathbb R) \,\;\quad\hat\otimes \;\cdots\; \hat\otimes \;\mathcal H_{\ell}(\mathbb R),
% \end{align*}
% where $\hat\otimes$ denotes the tensor product of Hilbert spaces.
% \item[C.] Using Equations \eqref{eqn:LB} and \eqref{eqn:UB} together with Proposition \ref{prop:Steinwart4.46}, we can conclude that
% \begin{align}
% \|\vA^* f\|_{\mathcal H_{\ell}(\mathbb R^d)} & = \bigg\|\sum_i g_i^1 \otimes \cdots \otimes g_i^d \bigg\|_{\mathcal H_\ell (\mathbb R) \hat\otimes \cdots \hat\otimes \mathcal H_\ell(\mathbb R)} \nonumber \\
% & \leq \left(\frac{\sqrt{\lambda_1}}{\ell}\right)^{\frac{1}{2}} \cdots \left(\frac{\sqrt{\lambda_d}}{\ell}\right)^{\frac{1}{2}} \bigg\|\sum_i g_i^1 \otimes \cdots \otimes g_i^d \bigg\|_{\mathcal H_{\lambda_1}(\mathbb R) \hat\otimes \cdots \hat\otimes \mathcal H_{\lambda_d}(\mathbb R)} \nonumber \\
% & \leq \left(\frac{U}{\ell}\right)^{\frac{d}{2}} \bigg\|\sum_i g_i^1 \otimes \cdots \otimes g_i^d \bigg\|_{\mathcal H_{\lambda_1}(\mathbb R) \hat\otimes \cdots \hat\otimes \mathcal H_{\lambda_d}(\mathbb R)} \nonumber \\
% & = \left(\frac{U}{\ell}\right)^{\frac{d}{2}} \|\vA^* f\|_{\mathcal H_{\mathbf{\vDelta}_d}(\mathbb R^d)}, \label{eqn:KernelShrink}
% \end{align}
% where the two inequalities are true with probability $1-\frac{\epsilon}{2}$ each, and so they both hold with probability $1-\epsilon$.
% \end{itemize}
% 
% Composing the Inequality \eqref{eqn:KernelShrink} with Equality \eqref{eqn:KernelIso} gives us the bound claimed in Inequality \eqref{eqn:RKHSNormBound}.
Now that we know that the $\mathcal H_{\ell}(\mathbb{R}^d)$ norm of $\vA^* f$ is finite, we can apply the Expected Improvement algorithm to it on the set $\vA^{-1}(\mathcal X)$ with kernel $k_\ell$, instead of the unknown kernel $k_{\vDelta_d}$, and then Proposition \ref{thm:Bull} tells us that the simple regret would be in $\mathcal O\big(t^{-\frac{1}{d}}\big)$.
\end{proof}


==> embedding_arxiv/secondproof.tex <==

\begin{proof}
Since $\mathcal{X}$ is a box constraint, by projecting $\vx^\star$ to $\cal T$ we get $\vx^\star_\top \in \mathcal{T} \cap \mathcal{X}$. Also, since $\vx^\star =  \vx^\star_\top + \vx_\bot$ for some $\vx_\bot \in \cal T^{\bot}$, we have $f(\vx^\star) = f(\vx^\star_\top)$. Hence, $\vx^\star_\top$ is an optimizer.
By using the same argument as appeared in Proposition 1, it is easy to see that with probability $1$ $\forall \vx \in \cal T$ $\exists \vy \in \mathbb{R}^d$ such that $\vA\vy = \vx + \vx_\bot$ where $\vx_\bot \in \cal T^{\bot}$. Let $\vPhi$ be the matrix whose columns form a standard basis for $\cal T$. Without loss of generality, we can assume that 
\[ \vPhi = \begin{bmatrix}\vI_{d_e} \\
\mathbf{0} \end{bmatrix} \]
Then, as shown in Proposition~\ref{prop:1}, there exists a $\vy^\star \in \mathbb{R}^d$ such that $\vPhi \vPhi^{T}\vA \vy^\star = \vx^\star_\top$. Note that for each column of $\vA$, we have
\[ \vPhi \vPhi^{T}\va_i \sim \mathcal{N}\left(\mathbf{0}, \begin{bmatrix}
\vI_{d_e} & {\bf 0}\\
{\bf 0} & {\bf 0}\end{bmatrix}\right). \]
Therefore $\vPhi \vPhi^{T}\vA\vy^\star = \vx^\star_\top$ is equivalent to $\vB\vy^\star = \bar{\vx}^\star_\top$ where $\vB\in \mathbb{R}^{d_e \times d_e}$ is a random matrix with independent standard Gaussian entries and $\bar{\vx}^\star_\top$ is the vector that contains the first $d_e$ entries of $\vx^\star_\top$ (the rest are $0$'s). By Theorem 3.4 of \cite{Sankar:2003}, we have
\[ \mathbb{P}\left[\|\vB^{-1}\|_2 \geq \frac{\sqrt{d_e}}{\epsilon}\right]  \leq \epsilon. \]

Thus, with probability at least $1-\epsilon$, $\|\vy^\star\| \leq \|\vB^{-1}\|_2  \|\bar{\vx}^\star_\top\|_2 = \|\vB^{-1}\|_2  \|\vx^\star_\top\|_2 \leq \frac{\sqrt{d_e}}{\epsilon} \|\vx^\star_\top\|_2$. 
\end{proof}


==> embedding_arxiv/theory.tex <==
%!TEX root = embedding.tex
Before introducing our new algorithm and its theoretical properties, we need to define what we mean by effective dimensionality formally.
\begin{mydefinition}\label{def:effdim}
A function $f: \mathbb{R}^{D} \rightarrow \mathbb{R}$ is said to have \textbf{effective dimensionality} $d_e$, with $d_e \leq D$, if 
\begin{itemize}
\denselist
	\item there exists a linear subspace ${\cal T}$ of dimension $d_e$ such that for all $\vx_{\top} \in {\cal T} \subset \mathbb{R}^D$ and $\vx_{\bot} \in {\cal T}^{\bot} \subset \mathbb{R}^D$, we have $f(\vx_{\top} + \vx_{\bot}) = f(\vx_{\top})$, where ${\cal T}^{\bot}$ denotes the orthogonal complement of ${\cal T}$; and
	\item $d_e$ is the smallest integer with this property.
\end{itemize}
We call ${\cal T}$ the \textbf{effective subspace} of $f$ and ${\cal T}^{\bot}$ the \textbf{constant subspace}.
\end{mydefinition}
\vspace{-2mm}
This definition simply states that the function does not change along the coordinates $\vx_{\bot}$, and this is why we refer
to ${\cal T}^{\bot}$ as the {constant subspace}.
Given this definition,
the following theorem shows that problems of low effective dimensionality can be solved via random embedding.

\begin{theorem}
\label{prop:1}
Assume we are given a function $f: \mathbb{R}^{D} \rightarrow \mathbb{R}$ with effective dimensionality $d_e$ and a random matrix $\vA \in \mathbb{R}^{D\times d}$ with independent entries sampled according to $\mathcal{N}(0, 1)$ and $d\geq d_e$. Then, with probability 1, for any $\vx \in \mathbb{R}^D$, there exists a $ \vy \in \mathbb{R}^d$ such that $f(\vx) = f(\vA\vy)$.
\end{theorem}
\vspace{-5mm}
\begin{proof}
Please refer to the appendix.
\end{proof}

Theorem~\ref{prop:1} says that given any $\vx \in \mathbb{R}^D$ and a random matrix $\vA \in \mathbb{R}^{D\times d}$, with probability $1$, there is a point $\vy \in \mathbb{R}^d$ such that $f(\vx) = f(\vA\vy)$. 
This implies that for any optimizer $\vx^{\star} \in \mathbb{R}^D$, there is a point $\vy^{\star} \in \mathbb{R}^d$ with $f(\vx^\star) = f(\vA\vy^{\star})$. Therefore, instead of optimizing in the high dimensional space, we can optimize the function $g(\vy) = f(\vA\vy)$ in the lower dimensional space.
This observation gives rise to our new Random EMbedding Bayesian Optimization (REMBO) algorithm (see Algorithm \ref{alg:embed}). REMBO first draws a random embedding (given by $\vA$) and then performs Bayesian optimization in this embedded space.
% computes a bounded region $\mathcal{Y}$ in the low-dimensional space, and 



\begin{algorithm}
\caption{REMBO: Bayesian Optimization with Random Embedding. Blue text denotes parts that are changed compared to standard Bayesian Optimization.}
\label{alg:embed}
\begin{algorithmic}[1]
{
\STATE \textcolor{blue}{Generate a random matrix $\vA \in \mathbb{R}^{D\times d}$}
\STATE \textcolor{blue}{Choose the bounded region set $\mathcal{Y} \subset \mathbb{R}^{d}$}
\STATE Initialize $\mathcal{D}_{0}$ as $\emptyset$.
\FOR{$t=1,2,\dots$}
  \STATE Find \textcolor{blue}{$\vy_{t+1} \in \mathbb{R}^d$} by optimizing the acquisition function $u$: \textcolor{blue}{$\vy_{t+1} = \argmax_{\vy\in \mathcal{Y}} u(\vy|\mathcal{D}_t).$} 
  \STATE Augment the data $\mathcal{D}_{t+1} = \mathcal{D}_{t} \cup \{ \textcolor{blue}{(\vy_{t+1}, f(\vA\vy_{t+1}))} \}$.
\STATE Update the kernel hyper-parameters.
\ENDFOR
}
\end{algorithmic}
\end{algorithm}


\begin{figure}[t]
\centering
  \includegraphics[scale=0.35]{figures/projection.pdf}
	% \note{FH: In this figure, can we change the text ``convex projection of $\vA\vy$ to $\mathcal{X}$'' to ``convex projection $p_{\mathcal{X}}(\vA\vy)$ of $\vA\vy$ to $\mathcal{X}$''
	% }
  \caption{Embedding from $d=1$ into $D=2$. The box illustrates the 2D constrained space ${\cal X}$, while the thicker red line illustrates the 1D constrained space $\mathcal{Y}$. Note that if $\vA\vy$ is outside $\mathcal{X}$, it is projected onto $\mathcal{X}$. The set $\mathcal{Y}$ must be chosen large enough so that the projection of its image, $\vA \mathcal{Y}$, onto the effective subspace (vertical axis in this diagram) covers the vertical side of the box.}
  \label{fig:proj}
\end{figure}

In many practical optimization tasks, the goal is to optimize $f$ over a compact subset $\mathcal{X} \subset \mathbb{R}^{D}$ (typically a box), and $f$ can often not be evaluated outside of $\mathcal{X}$. Therefore, when REMBO selects a point $\vy$ such that $\vA\vy$ is outside the box $\mathcal{X}$, it projects $\vA\vy$ onto $\mathcal{X}$ before evaluating $f$. That is, 
$g(\vy) = f(p_{\mathcal{X}}(\vA\vy))$, where $p_{\mathcal{X}}:\mathbb{R}^D \rightarrow \mathbb{R}^D$ is the standard projection operator for our box-constraint: $p_{\mathcal{X}}(\vy) = {\arg \min}_{\vz\in \mathcal{X}} \|\vz-\vy\|_2$; see Figure~\ref{fig:proj}.
%
We still need to describe how REMBO chooses the bounded region $\mathcal{Y} \subset \mathbb{R}^{d}$, inside which it performs Bayesian optimization. This is important because REMBO's effectiveness depends on the size of $\mathcal{Y}$. Locating the optimum within $\mathcal{Y}$ is easier if $\mathcal{Y}$ is small, but if we set $\mathcal{Y}$ too small it may not actually contain the global optimizer.
In the following theorem, we show that we can choose $\mathcal{Y}$ in a way that only depends on the effective dimensionality $d_e$ such that the optimizer of the original problem is contained in the low dimensional space with constant probability.

\begin{theorem}
\label{prop:2}
Suppose we want to optimize a function $f: \mathbb{R}^{D} \rightarrow \mathbb{R}$ with effective dimension $d_e \leq d$ subject to the box constraint $\mathcal{X} \subset \mathbb{R}^D$, where $\mathcal{X}$ is centered around $\mathbf{0}$. 
%Let us denote one of the optimizers by $\vx^{\star}$.
% \note{FH: dropped since unused: ``Let us denote one of the optimizers by $\vx^{\star}$.''}
Suppose further that the effective subspace $\cal T$ of $f$ is such that $\cal T$ is the span of $d_e$ basis vectors, and let $\vx^{\star}_\top \in \cal{T} \cap \mathcal{X}$ be an optimizer of $f$ inside $\mathcal{T}$. 
If $\vA$ is a $D\times d$ random matrix with independent standard Gaussian entries,
there exists an optimizer $\vy^\star \in \mathbb{R}^{d}$ such that $f(\vA\vy^\star) = f(\vx^\star_\top)$ and $\|\vy^\star\|_2 \leq \frac{\sqrt{d_e}}{\epsilon}\|\vx^{\star}_\top\|_2$ with probability at least $1-\epsilon$.
\end{theorem}
\vspace{-6mm}
\begin{proof}
Please refer to the appendix.
\end{proof}

Theorem~\ref{prop:2} says that if the set $\mathcal{X}$ in the original space is a box constraint, then there exists an optimizer $\vx^\star_\top \in \mathcal{X}$ that is $d_e$-sparse such that with probability at least $1-\epsilon$, $\|\vy^\star\|_2 \leq \frac{\sqrt{d_e}}{\epsilon}\|\vx^{\star}_\top\|_2$ where $f(\vA\vy^\star) = f(\vx^\star_\top)$. If the box constraint is $\mathcal{X} = [-1,1]^D$ (which is always achievable through rescaling), we have with probability at least $1-\epsilon$ that 
\[ \|\vy^\star\|_2 \leq \frac{\sqrt{d_e}}{\epsilon}\|\vx^{\star}_\top\|_2 \leq \frac{\sqrt{d_e}}{\epsilon}\sqrt{d_e}. \]
%\note{FH: fixed a typo. It said: $\|\vy^\star\|_2 \leq \frac{\sqrt{d}}{\epsilon}\|\vx^{\star}_\bot\|_2 \leq \frac{\sqrt{d}}{\epsilon}\sqrt{d}.$}
Hence, to choose $\mathcal{Y}$, we must ensure that the ball of radius $d_e/\epsilon$, centred at the origin, lies inside $\mathcal{Y}$. 

In practice, we have found that it is very unlikely that the optimizer falls on the corner of the box constraint,
implying that $\|x_{\top}^{\star}\| < \sqrt{d_e}$. Thus setting $\calY$ too big may
be unnecessarily wasteful. To improve our understanding of this effect, we developed a simulation study, in which we drew 
random Gaussian matrices, used them to map various potential optimizers $\vx^{\star}_\top$ to their corresponding points $\vy^{\star}_\top \in \calY$,
and studied the norms of $\vy^{\star}_\top$.

Assume for simplicity of presentation that $\calY$ is axis-aligned and $d_e$-dimensional (the argument applies when $d > d_e$). 
The section of the random matrix $\vA$ that maps points in $\calY$ to $\calT$ is a 
random Gaussian matrix of dimension $d_e\times d_e$. Let us call this section of 
the matrix $\vB$.
Since random Gaussian matrices are rotationally invariant in distribution, we have for any orthonormal matrix 
$\vO$ and a random Gaussian matrix $\vB$, $\vO\vB \,{\buildrel d \over =}\, \vB$. That is, $\vO\vB$ and $\vB$ are equal in distribution.
Similarly, for $\vB^{-1}$, 
$\vO\vB^{-1} = \left(\vB \vO^T\right)^{-1} \,{\buildrel d \over =}\, \vB^{-1}$. 
Therefore, $\vB^{-1}$
is also rotationally invariant. Hence, 
$\|\vB^{-1}\vx_{\top}\|_{\infty} \,{\buildrel d \over =}\, \|\vB^{-1}\vx'_{\top}\|_{\infty}$
as long as $\|\vx_{\top}\|_2 = \|\vx'_{\top}\|_2$. Following this equivalence for the supremum norm of projected vectors, it suffices to choose a point 
with the largest norm in $[-1, 1]^{d_e}$ in our simulations. We chose $\vx_{\top} = [1, 1, \cdots, 1]$.
 
We conducted simulations for several embedding dimensions, 
$d_e \in \{1, 2, \cdots, 50\}$, by drawing $10000$ random Gaussian
matrices and computing $\|\vB^{-1}\vx\|_{\infty}$.
We found that with empirical probability above $1-\epsilon$ (for decreasing values of $\epsilon$), it was the case that
$$\|\vB^{-1}\vx\|_{\infty} < \frac{1}{\epsilon} \max\{\log(d_e), 1\}.$$
These simulations indicate that we could set $\mathcal{Y} = \left[-\frac{1}{\epsilon} \max\{\log(d_e), 1\}, 
\frac{1}{\epsilon} \max\{\log(d_e), 1\}\right]^{d_e}$. We did this in our experiments and in particular chose $\epsilon =\log(d)/\sqrt{d}$, so that $\calY$ was $[-\sqrt{d}, \sqrt{d}]^d$. Note that Theorem~\ref{prop:2} is not useful for this choice, which suggests that there is room to improve this aspect of our theory.

% \textcolor{red} {
Some careful readers may wonder about the effect of the extrinsic dimensionality $D$. 
In the following theorem, we show that given the same intrinsic dimensions, 
the extrinsic dimensionality does not have an effect at all; in other words, REMBO is invariant to 
the addition of unimportant dimensions. 
\begin{theorem}[Invariance to addition of unimportant dimensions]
\label{prop:invar-D}
	Let $f: \mathbb{R}^{d_e} \rightarrow \mathbb{R}$ and for any $D \in \mathbb{N}$, $D \geq d_e$, define $f_{D}: \mathbb{R}^{D} \rightarrow \mathbb{R}$
	such that	$f_D$ adds $D-d_e$ truly unimportant dimensions to $f$: $f_{D}(\vz) = f(\vz_{1:d_e})$.
%	Let $\mathcal{Y}_D = [l_1,u_1] \times \cdots [l_D,u_D] \subset \mathbb{R}^{D}$ be a box constraint in $D$ dimensions for any $D \in \mathbb{N}$, $D \geq d_e$.
	Let $\vA_1 \in \mathbb{R}^{D_1\times d}$ and $\vA_0 \in \mathbb{R}^{(D_2-D_1)\times d}$ be random Gaussian matrices with $D_2 \geq D_1 \geq d$ and let
	$\vA_2 = 
	\begin{bmatrix}
	\vA_1\\
  \vA_0
	\end{bmatrix}.$
 %	$\vA_2 = [^\top \vA_0^\top]^\top$.
	Then, REMBO run using the same dimension $d \ge d_e$ and bounded region $\mathcal{Y}$
	yields exactly the same function values when run with $\vA_1$ on $f_{D_1}$ 
	as when run with $\vA_2$ on $f_{D_2}$.
	\end{theorem}
\begin{proof}
	We only need to show that for each $\vy \in \mathbb{R}^{d}$, we have $f_{D_1}( \vA_1 \vy ) = f_{D_2}( \vA_2 \vy )$
	since this step of REMBO (line 6 of Algorithm \ref{alg:embed}) is the only one that differs between the two algorithm runs. 
	When this function evaluation step yields the same results for every $\vy \in \mathbb{R}^{d}$, then
	the two REMBO runs behave identically since the algorithm is otherwise identical and deterministic after the selection of $\vA$ in Step 1.
%	
	Since 
	$\vA_2 = 
	\begin{bmatrix}
	\vA_1\\
  \vA_0
	\end{bmatrix}$, we have 
%
  $\vA_2 \vy = 
	\begin{bmatrix}
	\vA_1 \vy\\
  \vA_0 \vy
	\end{bmatrix}$.
%
	Since $D_2 \ge D_1 \ge d_e$, the first $d_e$ entries of this $D_2 \times 1$ vector $\vA_2 \vy$ are the first $d_e$ entries of $\vA_1 \vy$.
	We thus have 
	$f_{D_1}( \vA_1 \vy ) = f([\vA_1 \vy]_{1:d_e}) = f([\vA_2 \vy]_{1:d_e}) = f_{D_2}( \vA_2 \vy )$.
\end{proof}
% }	

% \textcolor{magenta} {
Finally, we show that REMBO is also invariant to rotations in the sense that
given different rotation matrices, running REMBO would result in the same distributions of observed function values. The argument is made concise in the following results.
\begin{lemma}
\label{lem:invar-rot}
	Consider function $f: \mathbb{R}^{D} \rightarrow \mathbb{R}$. 
	Let $f_{\vR}: \mathbb{R}^{D} \rightarrow \mathbb{R}$ be such that 
	$f_{\vR}(\vx) = f(\vR \vx)$ for some orthonormal matrix $\vR \in \mathbb{R}^{D \times D}$.
	Then, REMBO run in bounded region $\mathcal{Y}$
	yields exactly the same sequence of function values when run with $\vA$ on $f$ 
	as when run with $\vR^{-1} \vA$ on $f_{\vR}$ 
	for a matrix $\vA \in \mathbb{R}^{D\times d}$.
	\end{lemma}
\begin{proof}
	REMBO uses $f$ and $\vA$ (resp.\ $f_{\vR}$ and $\vR^{-1} \vA$) only in one spot (in line 6).
	Thus, the proof is trivial by showing that $f(\vA \vy_{t+1}) = f_{\vR}(\vR^{-1} \vA \vy_{t+1})$ through simple algebra:
	\[f_{\vR}(\vR^{-1} \vA \vy_{t+1}) = f(\vR \vR^{-1} \vA \vy_{t+1}) = f(\vA \vy_{t+1}).\]	
\end{proof}
\begin{theorem}[Invariance to rotations]
\label{prop:invar}
	Consider function $f: \mathbb{R}^{D} \rightarrow \mathbb{R}$. 
	Let $f_{\vR}: \mathbb{R}^{D} \rightarrow \mathbb{R}$ be such that 
	$f_{\vR}(\vx) = f(\vR \vx)$ for some orthonormal matrix $\vR \in \mathbb{R}^{D \times D}$.
	Then, given random Gaussian matrices $\vA_1 \in \mathbb{R}^{D\times d}$ 
	and $\vA_2 \in \mathbb{R}^{D\times d}$,
	REMBO run in bounded region $\mathcal{Y}$
	yields in distribution the same sequence of function values when run with $\vA_1$ on $f$ 
	as when run with $\vA_2$ on $f_{\vR}$.
\end{theorem}
\begin{proof}
	Since $\vR$ is orthonormal, we have $\vR^{-1} \vA_1 \overset{d}{=} \vA_2$.
	Therefore, REMBO run in bounded region $\mathcal{Y}$
	yields in distribution the same sequence of function values when run with $\vR^{-1} \vA_1$ on $f_{\vR}$ 
	as when run with $\vA_2$ on $f_{\vR}$.
	We have also by Lemma~\ref{lem:invar-rot} that REMBO run in bounded region $\mathcal{Y}$
	yields exactly the same sequence of function values when run with $\vA_1$ on $f$ 
	as when run with $\vR^{-1} \vA_1$ on $f_{\vR}$. The conclusion follows from combining the previous arguments.
\end{proof}
% }	

% \note{FH: I didn't touch the following theorem by Ziyu.}
% \textcolor{blue} {
% Finally, we show that REMBO is also invariant to rotations in the sense that
% given different rotation matrices, the constructed objective functions have the same 
% distribution. The argument is made concise in the following theorem.
% \begin{theorem}[Invariance to rotations]
% \label{prop:invar}
% 	Assume we are given a function $g: \mathbb{R}^{d_e} \rightarrow \mathbb{R}$.
% 	For any $D \in \mathbb{N}$, $D \geq d_e$, 
% 	define function $g_{D}: \mathbb{R}^{D} \rightarrow \mathbb{R}$ such that 
% 	$g_{D}(\vz) = g(\vz_{1:d_e})$
% 	and function $f^D_{\vR}: \mathbb{R}^{D} \rightarrow \mathbb{R}$ such that
% 	$f^D_{\vR}(\vx) = g_{D}(\vR \vx)$ for some orthonormal matrix 
% 	$\vR \in \mathbb{R}^{D \times D}$. 
% 	Then, given random Gaussian matrices $\vA_1 \in \mathbb{R}^{D\times d}$ 
% 	and $\vA_2 \in \mathbb{R}^{D\times d}$,
% 	$f^{D}_{\vR_1}(\vA_1 \vy) 
% 	\overset{d}{=} f^{D}_{\vR_2}(\vA_2 \vy)$ for any $D \geq d_e$,
% 	orthonormal matrices $\vR_1, \vR_2$, and $\vy \in \mathbb{R}^d$.
% \end{theorem}
% \begin{proof}
% 	Since we have that $\vR_1$ and $\vR_2$ are orthonormal, we have that
% 	$\vR_1 \vA_1$ and $\vR_2 \vA_2$ are also random matrices with independent Gaussian entries.
% 	The rest of the proof follows from simple algebra:
% 	$
% 		f^{D}_{\vR_1}(\vA_1 \vy) 
% 		= g_{D}(\vR_1 \vA_1 \vy) 
% 		\overset{d}{=} g_{D}(\vA_1 \vy)
% 		= g([\vA_1 \vy]_{1:d_e})  
% 		\overset{d}{=} g([\vA_2 \vy]_{1:d_e}) 
% 		= g_{D}(\vA_2 \vy)
% 		\overset{d}{=} g_{D}(\vR_2 \vA_2 \vy)
% 		 = f^{D}_{\vR_2}(\vA_2\vy).
% 	$
% \end{proof}
% }
% \note{FH: have you redone the experiments with this setting? If not we should state the setting used in the experiments.}

\subsection{Increasing the Success Rate of REMBO}\label{sec:increasing_rembo_success}

Theorem~\ref{prop:2} only guarantees that $\mathcal{Y}$ contains the optimum with probability at least $1-\epsilon$;
with probability $\delta \le \epsilon$ the optimizer lies outside of $\mathcal{Y}$. There are several ways to guard against this problem. One is to simply run REMBO multiple times with different independently drawn random embeddings. 
%
Since the probability of failure with each embedding is $\delta$, 
%and since failure events for independently sampled embeddings are independent, 
the probability of the optimizer not being included in the considered space of $k$ independently drawn embeddings is $\delta^k$. 
Thus, the failure probability vanishes exponentially quickly in the number of REMBO runs, $k$. 
Note also that these independent runs can be trivially parallelized to harness the power of
modern multi-core machines and large compute clusters.

%These $k$ runs can be trivially parallelized, and its has been demonstrated recently that performing multiple independent runs can yield high parallelization efficiency even for standard Bayesian optimization methods~\cite{HutHooLey12-ParallelAC}

%even multiple runs of standard Bayesian optimization are often sufficiently uncorrelated for this simple approach to achieve surprisingly high parallelization efficiency~\cite{HutHooLey12-ParallelAC}. Since REMBO runs with independently drawn embeddings are even less correlated, we expect REMBO to benefit even more from this parallelization approach, making it a promising method for harnessing the power of modern multi-core machines and large compute clusters.

%FH: this text might want to live in the intro, as a teaser of what lays ahead.
%Despite the extra runs required to lower the failure probability, REMBO is far more efficient than BO when the dimensionality gap $D-d$ is large and $d$ is low. While in this case we still have to run BO in $D$-dimensions, we only need to run REMBO in $d$-dimensions. As the experiments will show, one can easily (and effectively) run REMBO for $D=1\,000\,000\,000$ and $d=2$, but the same is not true for BO. Note also that repeated runs can be easily parallelized.

Another way of increasing REMBO's success rate is to increase the dimensionality $d$ it uses internally. When $d > d_e$, with probability $1$ we have ${ d \choose d_e }$ different embeddings of dimensionality $d_e$. 
That is,
we only need to select $d_e$ columns of $\vA \in \mathbb{R}^{D \times d}$ to represent the $d_e$ relevant dimensions of $\vx$.
The algorithm can achieve this by setting the remaining $d-d_e$ sub-components of the $d$-dimensional vector $\vy$ to zero. 
%The statement is probabilistic because the selection process is governed by the multiplication of the random matrix $\vA$ by $\vy$. 
Informally, since we have more embeddings, it is more likely that one of these will include the optimizer.
In our experiments, we will assess the merits and shortcomings of these two strategies. 

%We note that since REMBO only has to search a low-dimensional space, it converges far faster
%than standard BO in the original high-dimensional space. Thus, even in situations when REMBO's
%space does not contain the true optimizer it can yield much improved performance based on
%the small number of allowed function evaluations that is characteristic of most practical applications
%of Bayesian optimization.

\subsection{Choice of Kernel}\label{sec:choice_of_kernel}

Since REMBO uses GP-based Bayesian optimization to search in the region $\mathcal{Y} \subset \mathbb{R}^{d}$, 
we need to define a kernel between two points $\vy^{(1)}, \vy^{(2)} \in {\cal Y}$. 
We begin with the standard definition of the squared exponential kernel:
\begin{mydefinition} 
Let $K_{SE}(\vy) = \exp(-\|\vy\|^2/2)$.
Given a length scale $\ell > 0$, we define the corresponding {squared exponential} kernel as 
\[ k_{\ell}^d(\vy^{(1)},\vy^{(2)}) = K_{SE}\left(\frac{\vy^{(1)}-\vy^{(2)}}{\ell}\right) \]
% \exp\left({-\frac{\|\vy^{(1)}-\vy^{(2)}\|^2}{2\ell^2}}\right). \]
\label{def:sekernel}
\end{mydefinition}
\vspace{-3mm}
It is possible to work with two variants of this kernel. 
First, we can use $k_{\ell}^d(\vy^1, \vy^2)$ as in Definition~\ref{def:sekernel}. We refer to this kernel as the low-dimensional kernel. We can also adopt an implicitly defined high-dimensional kernel on 
$\mathcal{X}$:
$$k_{\ell}^D(\vy^{(1)}, \vy^{(2)}) = K_{SE}\left( \frac{p_{\mathcal{X}}(\vA\vy^{(1)}) - p_{\mathcal{X}}(\vA\vy^{(2)})}{\ell} \right),$$
where $p_{\mathcal{X}}:\mathbb{R}^D \rightarrow \mathbb{R}^D$ is the projection operator for our box-constraint as above (see Figure~\ref{fig:proj}). 


Note that when using this high-dimensional kernel, we are fitting the GP in $D$ dimensions. However, the search space is no longer the box $\mathcal{X}$, but it is instead given by the much smaller subspace $\{p_{\mathcal{X}}(\vA\vy): \vy \in {\cal Y} \}$. Importantly, in practice it is easier to maximize the acquisition function in this subspace.   

Both kernel choices have strengths and weaknesses. 
The low-dimensional kernel has the benefit of only requiring the construction of a GP in the space of intrinsic dimensionality $d$, whereas the high-dimensional kernel requires the GP to be constructed in a space of extrinsic dimensionality $D$.
%
However, the low-dimensional kernel may waste time exploring in the region of the embedding outside of ${\cal X}$ (see Figure 2) because two points far apart in this region may be projected via $p_{\mathcal{X}}$ to nearby points on the boundary of ${\cal X}$. The high-dimensional kernel is not affected by this problem because the search is conducted directly on $\{p_{\mathcal{X}}(\vA\vy): \vy \in {\cal Y} \}$ with distances calculated in $\cal X$ and not in $\cal Y$. 
 

The choice of kernel also depends on whether our variables are continuous, integer or categorical. The categorical case is important because we often encounter optimization problems that contain discrete choices. We define our kernel for categorical variables as:
% \note{FH: I reworded the following; please check.}
$$k^D_{\lambda}(\vy^{(1)}, \vy^{(2)}) = \exp\left(-\frac{\lambda}{2} h(s(\vA\vy^{(1)}), s(\vA\vy^{(2)}))^2 \right),$$
where $\vy^{(1)}, \vy^{(2)} \in {\cal Y} \subset \mathbb{R}^d$,
the function $s$ maps continuous $d$-dimensional vectors to discrete $D$-dimensional vectors, and 
$h$ defines the distance between two discrete vectors. In more detail, $s(\vx)$ first uses $p_{\mathcal{X}}$ to  project $\vx$ to $\bar{\vx} \in [-1,1]^D$. For each dimension $\bar{x}_i$ of $\bar{\vx}$, $s$ then maps $\bar{x}_i$ to a discrete value by scaling and rounding. 
%\note{FH: should we give the formula for this scaling and rounding?}
In our experiments, following~\citeA{Hutter:2009}, we defined $h(\vx^{(1)}, \vx^{(2)}) = |\{i: x^{(1)}_i \neq x^{(2)}_i\}|$ 
%to deal with the categorical parameters 
so as not to impose an artificial ordering between the values of categorical parameters. 
%\note{FH: I believe that formula needs to be adapted to reflect that all distances are now always measured in the high-dim space (including the continuous parameters)? Also, if this section applies to continuous parameters just as well we should make that more clear.}
In essence, we measure the distance between two points in the low-dimensional space as the Hamming distance between their mappings in the high-dimensional space. 



==> journal-length-abstract-and-intro.tex <==
\begin{abstract}

Bayesian optimization is a powerful strategy for finding the extrema of objective functions. It is applicable in situations where one does not have a closed-form expression for the objective function, but where one can obtain noisy evaluations of this function at sampled values. It is particularly useful when these evaluations are costly, when one does not have access to derivatives, or when the problem at hand is non-convex. Bayesian optimization techniques have been successfully applied to robotics, planning, sensor placement, news recommendation, advertising, intelligent user interfaces and automatic algorithm configuration. Despite these successes, the approach is restricted to problems of moderate dimension. Several machine learning workshops on this topic have identified the scaling of Bayesian optimization to high-dimensions as a core challenge. Despite this, little progress has been made in this direction.
In this paper, we introduce a novel random embedding idea to scale Bayesian optimization to higher dimensions. The resulting algorithm is very simple, it has theoretical guarantees, it applies to domains with both categorical and continuous variables, and its hyper-parameters are automatically tuned. We show that the algorithm can effectively solve problems with billions of dimensions, provided the intrinsic dimensionality is low. We also show that it has important invariance properties. In terms of applications, we demonstrate that the algorithm performs remarkably well in the domains of automatic tuning of popular linear programming solvers and random forests classifiers for big data produced by the Kinect sensor.
\end{abstract}


\section{Introduction}
\label{sec:introduction}

Let $f: {\cal X} \to \mathbb{R}$ be a function on a compact subset ${\cal X} \subseteq \mathbb{R}^D$. We address the following global optimization problem
\[ \vx^{\star} = \argmax_{\vx \in {\cal X}} f(\vx). \]
We are particularly interested in objective functions $f$ that may satisfy any of the following criteria: Do not have a closed-form expression, are expensive to evaluate, are stochastic, do not have derivatives available, or are non-convex. For these reasons, we adopt the Bayesian optimization framework. We present a brief introduction to Bayesian optimization in this paper, but refer readers unfamiliar with the topic to more tutorial treatments \cite{Brochu:2009,Jones:1998,Jones:2001,Lizotte:2011,Mockus:1994,Osborne:2009}. 

Bayesian optimization has two ingredients. The first ingredient is a prior distribution that captures our beliefs about the behavior of the unknown objective function. The second ingredient is a risk function that describes the deviation from the global optimum. The expected risk is used to decide where to sample next. After observing a few samples of the objective, the prior is updated to produce a more informative posterior distribution over the space of objective functions \cite[see Figure 1 in][]{Brochu:2009}. One problem with this maximum expected utility framework is that the risk is typically very hard to compute. This has led to the introduction of many sequential heuristics, known as acquisition functions, including Thompson sampling \cite{Thompson:1933}, probability of improvement \cite{Jones:2001}, expected improvement \cite{Mockus:1994} and upper-confidence-bounds \cite{Srinivas:2010}. These acquisition functions trade-off exploration and exploitation. They are typically optimized by choosing points 
where the predictive mean is high (exploitation) and where the variance is large (exploration). Since the acquisition function has an analytical expression that is easy to evaluate, it is much easier to optimize than the original objective function, using algorithms such as DIRECT \cite{Finkel:2003} or projected Newton methods \cite{Bertsekas:1987}. It is also possible to use dynamic portfolios of acquisition functions to improve the efficiency of the method \cite{Hoffman:2011}. 

The term Bayesian optimization seems to have been coined several decades ago by Jonas Mo{\v c}kus \yrcite{Mockus:1982}. A popular version of the method has been known as efficient global optimization in the experimental design literature since the nineties \cite{Schonlau:1998}. Often, the approximation of the objective function is obtained using Gaussian process~(GP) priors. For this reason, the technique is also referred to as GP bandits \cite{Srinivas:2010}. However, many other approximations of the objective have been proposed, including Parzen estimators \cite{Bergstra:2011}, Bayesian parametric models \cite{Wang:2011}, treed GPs \cite{Gramacy:2004} and random forests \cite{Brochu:2009,Hutter:2009}. 
These may be more suitable than GPs when the number of iterations grows without bound, or when the objective function is believed to have discontinuities. We also note that often assumptions on the smoothness of the objective function are encoded without use of the Bayesian paradigm, while leading to similar algorithms and theoretical guarantees \cite[see, for example,][and the references therein]{Bubeck:2011,deFreitas:2012}.

In recent years, the machine learning community has increasingly used Bayesian optimization to optimize expensive objective functions. Despite many success stories, the approach is restricted to problems of moderate dimension, typically up to about 10. Of course, for a great many problems this is all that is needed. However, to advance the state of the art, we need to scale the methodology to high-dimensional parameter spaces. This is the goal of this paper.

It is difficult to scale Bayesian optimization to high dimensions. To ensure that a global optimum is found, we require good coverage of $\mathcal{X}$, but as the dimensionality increases, the number of evaluations needed to cover $\mathcal{X}$ increases exponentially. As a result, there has been little progress on this challenging problem, with a few exceptions.
%
%\note{NdF: Possibly revisit the following remark after experiments}
\citeA{Hutter:2011} used random forests models in Bayesian optimization to optimize up to 76 mixed discrete/continuous parameters of algorithms for solving hard combinatorial problems, empirically outperforming all competing algorithm configuration methods. However, their method is based on frequentist uncertainty estimates that can fail even for the optimization of very simple functions and lacks theoretical guarantees. Their software, which we benchmark against in our experiments, was the result of perhaps the most significant and non-trivial engineering endeavor in practical Bayesian optimization.
% the RFs are also axis-aligned, but that'll be better to mention in the context of the synthetic data experiment

In the \emph{linear} bandits case, \citeA{Carpentier:2012} recently proposed a compressed sensing strategy to attack problems with a high degree of sparsity. 
Also recently, Chen et al \citeA{Chen:2012} made significant progress by introducing a two stage strategy for optimization and variable selection of high-dimensional GPs. In the first stage, sequential likelihood ratio tests, with a couple of tuning parameters, are used to select the relevant dimensions. 
\note{FH: do we need ``with a couple of tuning parameters'' here? Seems to have a negative co-notation?}
This, however, requires the relevant dimensions to be axis-aligned with an ARD kernel. Chen et al provide empirical results only for synthetic examples (of up to 400 dimensions), but they provide key theoretical guarantees.

Many researchers have noted that for certain classes of problems most dimensions do not change the objective function significantly; examples include hyper-parameter optimization for neural networks and deep belief networks~\cite{Bergstra:2012} and automatic configuration of state-of-the-art algorithms for solving $\mathcal{NP}$-hard 
%problems~\cite{Hutter:2009}.
problems~\cite{Hutter:2013_key_parameters}.
%, and XXX~\cite{Caflisch:1997}. 
%\note{FH: TODO: what is the application domain in \cite{Caflisch:1997}??}
That is to say these problems have \emph{``low effective dimensionality''}. To take advantage of this property, \citeA{Bergstra:2012} proposed to simply use random search for optimization -- the rationale being that points sampled uniformly at random in each dimension can densely cover each low-dimensional subspace. As such, random search can exploit low effective dimensionality \emph{without knowing which dimensions are important}. In this paper, we exploit the same property in a new Bayesian optimization variant based on random embeddings. 
%In this paper, we show that random embeddings have the same property, and combine them with powerful Bayesian optimization in the low-dimensional subspace.


\begin{figure}[tb]
  \includegraphics[scale=0.16]{figures/2to1embedding.pdf}
  \centering
  \caption{This function only has one \emph{effective dimension}: the vertical axis indicated with the word important on the right hand side figure. Hence, the $1$D embedding includes the $2$D function's optimizer. It is more efficient to search for the optimum along the 1D random embedding than to conduct a grid-search in 2D.}
  \label{fig:simple_embedding}
\end{figure}

Figure \ref{fig:simple_embedding} illustrates the idea behind random embeddings in a nutshell.
Assume we know that a given $D=2$ dimensional black-box function $f(x_1, x_2)$ only has $d=1$ important dimensions, but we do not know which of the two dimensions is the important one.
We can then perform optimization in the embedded 1-dimensional subspace defined by $x_1=x_2$ since this is guaranteed to include the optimum. 
As we demonstrate in this paper, using random embeddings this simple idea largely scales to arbitrary $D$ and $d$, allowing us to perform
Bayesian optimization in a low-dimensional space to optimize a high-dimensional function with low intrinsic dimensionality.
Importantly, this trick is not restricted to cases with axis-aligned intrinsic dimensions but applies to any $d$-dimensional linear subspace.

After defining GP-based Bayesian optimization (Section \ref{sec:bo}), we describe Bayesian optimization based on random embeddings (REMBO) more formally and prove theoretical properties including regret bounds independent of $D$ (Section \ref{sec:rembo}). Then we demonstrate REMBO's empirical performance in a wide variety of settings (Section \ref{sec:experiments}). First, we evaluate scaling behaviour on synthetic data, demonstrating that REMBO can effectively optimize functions of low effective dimensionality embedded in a billion dimensions. Then, we demonstrate state-of-the-art performance for two real-world application domains: optimizing the 14 continuous parameters of a random forest classifier for body part classification using the Kinect sensor; and the 47 discrete parameters of a widely-used algorithm for solving mixed integer programs. 
%Section \ref{sec:conclusion} concludes the paper and points out promising directions for future work.


==> linearProg_old.tex <==
State-of-the-art algorithms for solving hard computational problems tend to parameterize several design choices in order to allow a customization of the algorithm to new problem domains. Automated methods for algorithm configuration have recently demonstrated that substantial performance gains of state-of-the-art algorithms can be achieved in a fully automated fashion~\cite{Mockus:1999,Hutter:2010,Bergstra:2011,Wang:2011}. These successes have led to a paradigm shift in algorithm development towards the active design of highly parameterized code followed by automated procedures to best instantiate this code for a given problem domain~\cite{Hoos:2012:PO:2076450.2076469,Bergstra:model_search}.

It has long been suspected that these algorithm configuration problems have low dimensionality~\cite{Hutter:2009}. Here, we demonstrate that REMBO can exploit this low dimensionality even in the discrete spaces typically encountered in algorithm configuration. 
We use a configuration problem obtained from \citeA{Hutter:2010}, aiming to configure the 40 binary and 7 categorical parameters of \text{lpsolve}\footnote{http://lpsolve.sourceforge.net/}, a popular mixed integer linear programming solver that has been downloaded over 40\,000 times in the last year.
The objective is to minimize the optimality gap \texttt{lpsolve} can obtain in a fixed time limit of five seconds for a mixed integer programming (MIP) encoding of a wildlife corridor problem from computational sustainability~\cite{ghs08:connection}.
Algorithm configuration usually aims to improve performance for a representative set of problem instances, and effective methods need to solve two orthogonal problems: searching the parameter space effectively and deciding how many instances to use in each evaluation (to trade off computational overhead and over-fitting). Our contribution is for the first of these problems; to focus on how effectively different methods search the parameter space, we only consider configuration on a single problem instance.

Due to the discrete nature of this optimization problem, we could only apply REMBO using the high-dimensional kernel for categorical variables $k^D_{\lambda}(\vy^{(1)}, \vy^{(2)})$ described in Section \ref{sec:choice_of_kernel}. While we have not proven any theoretical guarantees for discrete optimization problems, REMBO appears to effectively exploit the low effective dimensionality of this particular optimization problem.

\begin{figure}[tb]
\begin{center}
  \includegraphics[scale=0.35]{figures/lpsolve.png}\\
  \includegraphics[scale=0.35]{figures/lpsolve_interleave.png}
  \caption{Performance of various methods for configuration of \texttt{lpsolve}; we show the optimality gap \texttt{lpsolve} achieved with the configurations found by the various methods (lower is better). Top: a single run of each method; Bottom: performance with $k=4$ interleaved runs.}
\end{center}
\vspace*{-2mm}
\label{fig:lpsolve} 
\end{figure}


Figure \ref{fig:lpsolve} (top) compares BO, REMBO, and the baseline random search against the configuration procedures ParamILS (which was used for all configuration experiments in~\cite{Hutter:2010}),
%ParamILS~\cite{ParamILS-JAIR} (which was used for all configuration experiments in~\cite{Hutter:2010}), 
and SMAC \cite{Hutter:2011}. ParamILS and SMAC have been specifically designed for the configuration of algorithms with many parameters and define the current state of the art for this problem. As the figure shows, they indeed outperformed both BO and random search by a comfortable margin. However, remarkably, our vanilla REMBO method performed even slightly better. While the figure only shows REMBO with $d=5$ to avoid clutter, we by no means optimized this parameter; the only other value we tried was $d=3$, which resulted in indistinguishable performance. 

As in the synthetic experiment, REMBO's performance could be further improved by using multiple interleaved runs.
However, it is known that multiple independent runs can also improve the performance of the other procedures, especially ParamILS~\cite{HutHooLey12-ParallelAC}. Thus, to be fair, we re-evaluated all approaches using interleaved runs. Figure \ref{fig:lpsolve} (bottom) shows that when using $k=4$ interleaved runs of $500$ evaluations each, REMBO and ParamILS performed best, with a slight advantage for REMBO early on in the search.


%\note{FH: Ziyu, to get confidence in the wider applicability of this result, I'd like to do some additional experiments on more instances. Let's talk about them...}






==> randomForests.tex <==
%\note{FH: I was somewhat confused when I read this section the first time; Nando, since you know the domain well could you maybe have a look?}

The work of Shotton et al. \cite{Shotton:2011} demonstrated state-of-the-art real-time human pose estimation from depth images by classifying each pixel with a body part class.  The ground truth body part labels and corresponding depth image are visualized in Figure \ref{fig:rf-all}~(left). Following Shotton et al \cite{Shotton:2011}, the random forest classifier is trained with synthetic data.  Pairs of depth and labeled images are generated using open datasets and graphics packages. For this experiment, we used random poses from the CMU mocap database to generate two hundred pairs of 320x240 resolution depth and body part images.  

The feature space is the difference of depth between pairs of pixels.  The location of each pixel in the pair is specified as an offset from the pixel being classified. The center diagram of Figure \ref{fig:rf-all} shows one feature for the pixel in the green box.  The pixel location in the red box is specified by offset u and the pixel in the white box is specified by offset v.  By scaling the offsets u,v by the depth of the pixel being classified, the features are depth invariant.  The two offsets and threshold make up the five parameters of each node in the tree.  
%\note{FH: I guess an offset has two coordinates? In that case, I'd replace ``specified by offset u'' by ``specified by the 2-dimensional offset u'' for clarity.}
The tree is built using the standard approach of recursively constructing each node by selecting the offsets and threshold that maximizes the information gain; see \cite{Shotton:2011}
for more details.

Candidate offsets are drawn from a 2d Gaussian.  If the variance is low then the random forest classifier is learning local features.  If the variance is the high, the classifier is learning global features.  The candidate Gaussians for u and v are parameterized independently along with 4 other hyper parameters resulting in a total of 14 hyper-parameters.  The ranges for each parameter can be found in Table \ref{table:rf}.

For these experiments, the random forest classifier was trained from 100\,000 random pixels from the 140 pose training set. Including the background class, there were 5\,000 samples per body part class.  The random forest accuracy across all 4.6 million pixels in a 60 pose test set is plotted in the right of Figure~\ref{fig:rf-all}. 
Random search performed remarkably well at this task, clearly outperforming pure BO. However, REMBO performed yet better than Random. More importantly, REMBO found a parameter configuration that performed better than previous manual tuning.    
%\note{FH: Dave, could one say that that manual tuning was really tedious (optimally quantify the human time spent) or was done by experts, or matters a lot in practice? That would make this argument stronger...}


\begin{table}[t]
\caption{Hyperparameter ranges for random forest classifier}
\label{table:rf}
\begin{center}
{\footnotesize
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf Parameter}  &\multicolumn{1}{c}{\bf Range}
\\ \hline \\
Number of candidate offsets at each node         &[5 1000] \\
Minimum samples for non-leaf nodes             &[1 50] \\
Maximum depth of the tree             &[2 20] \\
Number of trees in forest             &[1 10] \\
X, Y mean of candidate offsets             &[-200 200]\\
X, Y and XY variance  of candidate offsets           &[0.0 300]\\
\end{tabular}
}
\end{center}
\vspace{-1.5em}
\end{table}

%\note{FH: Dave, are all the samples treated as lying on a uniform scale, or are some log-transformed? E.g. `Number of candidate offsets to try at each node' or `Minimum samples for non-leaf nodes'?}


\begin{figure}[t]
\centering
  \raisebox{0.6cm}{\includegraphics[height=0.2\textheight]{figures/rf-all-nips-cropped.png}} \vspace{0.25em}
  \raisebox{0.6cm}{\includegraphics[height=0.2\textheight]{figures/rf-all-nips-offsets.png}} \vspace{0.25em}
     \includegraphics[scale=0.38]{figures/rf.png}
  \caption{Ground truth depth, ground truth body parts and predicted body parts (left), features specified by offsets u and v (middle) and the plot of prediction accuracy (right).  REMBO selected better hyperparameter settings than both Random and Random.}
  \label{fig:rf-all}
\end{figure}

